Kinematics of the Orion Nebula Cluster: Velocity Substructure and Spectroscopic Binaries

We present a kinematic study of the Orion Nebula Cluster based upon radial velocities measured by multi-fiber echelle spectroscopy at the 6.5 meter MMT and Magellan telescopes. Velocities are reported for 1613 stars, with multi-epoch data for 727 objects as part of our continuing effort to detect and analyze spectroscopic binaries. We confirm and extend the results of Furesz et al. showing that the ONC is not relaxed, consistent with its youth, and that the stars generally follow the position-velocity structure of the moderate density gas in the region, traced by $^{13}$CO. The additional radial velocities we have measured enable us to probe some discrepancies between stellar and gaseous structure which can be attributed to binary motion and the inclusion of non-members in our kinematic sample. Our multi-epoch data allow us to identify 89 spectroscopic binaries; more will be found as we continue monitoring. Our results reinforce the idea that the ONC is a cluster in formation, and thus provides a valuable testing ground for theory. In particular, our observations are not consistent with the quasi-equilibrium or slow contraction models of cluster formation, but are consistent with cold collapse models.

==> tab10-full.tex <==
\begin{deluxetable}{lll}
\rotate
\tablewidth{0pt}

\tabletypesize{\scriptsize}
\tablecaption{MIKE Field D Velocity Data}
\tablehead{
  \colhead{2massID} &  \colhead{RV D\_1}  & \colhead{R D\_1}   \\
    \colhead{}    &  \colhead{(km s$^{-1}$)} &  \\

   }
\startdata
0534435-045136 & 36.9 $\pm$ 3.9  & 4.2  \\ 
0534441-044751 & 10.6 $\pm$ 3.3  & 5.1  \\ 
0534452-044758 & 33.2 $\pm$ 1.9  & 10.3  \\ 
0534494-044539 & 37.9 $\pm$ 1.0  & 25.4  \\ 
0534512-044757 & 35.7 $\pm$ 2.0  & 9.5  \\ 
0534520-045501 & 172.0 $\pm$ 4.0  & 4.1  \\ 
0534531-044310 & 27.7 $\pm$ 3.7  & 4.5  \\ 
0534538-045622 & 30.9 $\pm$ 1.3  & 17.2  \\ 
0534550-044941 & 29.2 $\pm$ 2.9  & 6.0  \\ 
0534551-044827 & 28.6 $\pm$ 1.0  & 24.9  \\ 
0534568-044604 & 32.2 $\pm$ 1.7  & 11.6  \\ 
0534574-045645 & -157.7 $\pm$ 4.1  & 4.0  \\ 
0534579-044912 & 29.0 $\pm$ 1.4  & 15.0  \\ 
0534593-045011 & 28.9 $\pm$ 2.0  & 9.3  \\ 
0535009-044818 & 28.5 $\pm$ 2.9  & 6.1  \\ 
0535019-044114 & 163.7 $\pm$ 4.3  & 3.7  \\ 
0535023-044916 & 31.0 $\pm$ 4.4  & 3.6  \\ 
0535030-044416 & 18.4 $\pm$ 4.1  & 3.9  \\ 
0535033-045643 & 29.3 $\pm$ 2.2  & 8.4  \\ 
0535048-044708 & 64.3 $\pm$ 4.4  & 3.6  \\ 
0535058-044843 & 30.4 $\pm$ 1.5  & 13.5  \\ 
0535069-044909 & 29.8 $\pm$ 2.4  & 7.6  \\ 
0535070-045456 & 30.7 $\pm$ 1.2  & 17.8  \\ 
0535079-043907 & 10.8 $\pm$ 0.9  & 29.9  \\ 
0535086-044652 & 36.6 $\pm$ 2.1  & 9.0  \\ 
0535093-044202 & 27.1 $\pm$ 2.4  & 7.5  \\ 
0535100-045108 & 29.1 $\pm$ 2.8  & 6.4  \\ 
0535108-044602 & 28.7 $\pm$ 2.0  & 9.3  \\ 
0535109-044712 & 23.5 $\pm$ 3.0  & 5.8  \\ 
0535115-044633 & 25.4 $\pm$ 2.3  & 7.9  \\ 
0535125-045155 & 33.2 $\pm$ 1.5  & 13.7  \\ 
0535130-044305 & 31.9 $\pm$ 3.3  & 5.1  \\ 
0535143-045522 & 24.4 $\pm$ 2.5  & 7.3  \\ 
0535156-045713 & 30.2 $\pm$ 3.6  & 4.6  \\ 
0535164-045802 & 29.9 $\pm$ 4.5  & 3.5  \\ 
0535172-044113 & 20.4 $\pm$ 3.2  & 5.4  \\ 
0535178-044452 & 29.1 $\pm$ 1.5  & 13.7  \\ 
0535183-045030 & 35.9 $\pm$ 2.8  & 6.4  \\ 
0535188-044410 & -61.7 $\pm$ 4.0  & 4.1  \\ 
0535189-045050 & -27.7 $\pm$ 0.9  & 27.0  \\ 
0535191-044349 & 30.6 $\pm$ 1.8  & 11.1  \\ 
0535192-044851 & 29.2 $\pm$ 2.4  & 7.8  \\ 
0535197-044818 & -131.7 $\pm$ 3.7  & 4.5  \\ 
0535201-044134 & 167.1 $\pm$ 4.5  & 3.5  \\ 
0535210-044538 & 31.3 $\pm$ 3.5  & 4.8  \\ 
0535214-044725 & 28.7 $\pm$ 3.8  & 4.3  \\ 
0535215-045045 & 30.9 $\pm$ 0.8  & 35.5  \\ 
0535216-044412 & 28.1 $\pm$ 4.2  & 3.9  \\ 
0535216-045648 & 25.8 $\pm$ 3.3  & 5.2  \\ 
0535217-045311 & 27.8 $\pm$ 0.8  & 32.6  \\ 
0535218-045019 & 25.5 $\pm$ 1.8  & 10.5  \\ 
0535218-045407 & 30.2 $\pm$ 1.9  & 10.4  \\ 
0535223-044207 & 30.4 $\pm$ 1.2  & 17.5  \\ 
0535228-044641 & 36.6 $\pm$ 3.4  & 5.0  \\ 
0535232-044302 & 20.0 $\pm$ 3.9  & 4.2  \\ 
0535233-045720 & 30.6 $\pm$ 1.8  & 10.8  \\ 
0535237-044346 & 24.4 $\pm$ 1.4  & 14.5  \\ 
0535237-044816 & 35.5 $\pm$ 3.4  & 5.0  \\ 
0535240-044515 & -0.3 $\pm$ 1.0  & 25.3  \\ 
0535241-045008 & 35.0 $\pm$ 3.5  & 4.7  \\ 
0535244-044456 & 3.8 $\pm$ 1.7  & 11.6  \\ 
0535254-045403 & 24.6 $\pm$ 2.1  & 8.9  \\ 
0535256-045718 & 6.5 $\pm$ 3.8  & 4.4  \\ 
0535265-045606 & 16.9 $\pm$ 3.5  & 4.7  \\ 
0535268-044730 & 24.1 $\pm$ 1.0  & 23.8  \\ 
0535276-045219 & 33.1 $\pm$ 4.2  & 3.8  \\ 
0535279-045133 & -32.1 $\pm$ 4.0  & 4.0  \\ 
0535286-045503 & 75.2 $\pm$ 2.8  & 6.2  \\ 
0535289-044913 & 26.1 $\pm$ 4.2  & 3.8  \\ 
0535303-045042 & 29.8 $\pm$ 0.9  & 27.3  \\ 
0535305-045128 & 29.7 $\pm$ 1.3  & 17.1  \\ 
0535306-043900 & 35.4 $\pm$ 3.6  & 4.7  \\ 
0535315-045343 & -9.5 $\pm$ 3.5  & 4.8  \\ 
0535324-045202 & 31.1 $\pm$ 1.3  & 15.9  \\ 
0535327-045011 & 30.4 $\pm$ 1.6  & 12.8  \\ 
0535329-044521 & 54.8 $\pm$ 1.3  & 16.0  \\ 
0535330-044358 & 30.1 $\pm$ 1.1  & 21.5  \\ 
0535333-045111 & 34.6 $\pm$ 4.2  & 3.9  \\ 
0535336-044623 & 33.5 $\pm$ 2.4  & 7.8  \\ 
0535340-045411 & 20.8 $\pm$ 2.7  & 6.7  \\ 
0535342-044953 & 28.3 $\pm$ 1.0  & 22.4  \\ 
0535344-044020 & 31.4 $\pm$ 2.5  & 7.1  \\ 
0535352-044739 & 32.2 $\pm$ 1.9  & 10.4  \\ 
0535355-045226 & 21.6 $\pm$ 1.3  & 15.9  \\ 
0535364-050115 & 32.4 $\pm$ 4.4  & 3.6  \\ 
0535375-044755 & 55.6 $\pm$ 0.8  & 33.3  \\ 
0535380-044833 & 33.5 $\pm$ 3.2  & 5.5  \\ 
0535385-045941 & 24.4 $\pm$ 1.1  & 19.5  \\ 
0535393-044734 & 80.1 $\pm$ 1.3  & 16.4  \\ 
0535394-044019 & 35.3 $\pm$ 3.5  & 4.9  \\ 
0535397-045021 & 15.2 $\pm$ 0.8  & 32.7  \\ 
0535397-045141 & 19.8 $\pm$ 0.9  & 27.1  \\ 
0535398-044404 & 30.9 $\pm$ 1.8  & 10.6  \\ 
0535400-044555 & 28.6 $\pm$ 1.2  & 17.9  \\ 
0535402-045106 & -3.3 $\pm$ 1.1  & 20.5  \\ 
0535404-045543 & 79.9 $\pm$ 4.4  & 3.6  \\ 
0535407-044830 & 24.3 $\pm$ 0.9  & 29.2  \\ 
0535410-044947 & 26.9 $\pm$ 1.4  & 14.7  \\ 
0535432-044247 & 27.6 $\pm$ 0.9  & 27.3  \\ 
0535441-044804 & 29.8 $\pm$ 2.7  & 6.7  \\ 
0535447-050039 & -45.1 $\pm$ 4.3  & 3.7  \\ 
0535451-044925 & 9.6 $\pm$ 0.9  & 27.7  \\ 
0535453-044339 & 32.0 $\pm$ 2.4  & 7.7  \\ 
0535456-044528 & 17.2 $\pm$ 0.9  & 30.9  \\ 
0535480-045020 & 25.4 $\pm$ 2.8  & 6.3  \\ 
0535484-050128 & -59.1 $\pm$ 4.2  & 3.8  \\ 
0535508-045111 & -6.6 $\pm$ 1.0  & 25.3  \\ 
0535517-045208 & 142.5 $\pm$ 3.2  & 5.5  \\ 
0535518-045410 & 22.3 $\pm$ 1.1  & 20.1  \\ 
0535522-044304 & 24.7 $\pm$ 2.1  & 9.2  \\ 
0535532-044734 & 27.1 $\pm$ 1.3  & 16.2  \\ 
0535538-045714 & 22.3 $\pm$ 4.0  & 4.1  \\ 
0535544-044804 & 29.0 $\pm$ 1.4  & 15.2  \\ 
0535547-045819 & 26.0 $\pm$ 2.7  & 6.6  \\ 
0535555-044440 & -14.5 $\pm$ 2.5  & 7.2  \\ 
0535560-045655 & 25.9 $\pm$ 1.2  & 19.3  \\ 
0535582-044643 & 25.8 $\pm$ 1.1  & 20.3  \\ 
0535583-045536 & 28.8 $\pm$ 2.6  & 7.0  \\ 
0535587-044300 & 76.6 $\pm$ 2.7  & 6.5  \\ 
0535592-045846 & 30.2 $\pm$ 1.7  & 11.7  \\ 
0536006-045606 & 10.2 $\pm$ 1.4  & 15.1  \\ 
0536008-044258 & 175.7 $\pm$ 4.3  & 3.7  \\ 
0536014-044341 & 54.6 $\pm$ 2.7  & 6.7  \\ 
0536033-045018 & 54.9 $\pm$ 0.9  & 28.6  \\ 
0536033-045740 & 102.4 $\pm$ 4.5  & 3.5  \\ 
0536039-044721 & 90.4 $\pm$ 1.2  & 19.0  \\ 
0536043-044439 & -5.5 $\pm$ 2.1  & 8.7  \\ 
0536044-045732 & -170.3 $\pm$ 4.1  & 4.0  \\ 
0536053-045316 & 23.8 $\pm$ 0.9  & 26.4  \\ 
0536055-044854 & -8.0 $\pm$ 1.1  & 21.9  \\ 
0536064-044153 & 25.9 $\pm$ 2.6  & 7.0  \\ 
0536079-044940 & 45.9 $\pm$ 1.7  & 11.4  \\ 
0536090-044935 & 81.8 $\pm$ 2.0  & 9.8  \\ 
0536092-045000 & 78.4 $\pm$ 4.1  & 3.9  \\ 
0536130-045513 & 30.1 $\pm$ 3.8  & 4.4  \\ 
0536144-045015 & -35.5 $\pm$ 1.0  & 23.5  \\ 
\enddata
\end{deluxetable}


==> tab4-full.tex <==
\begin{deluxetable}{lllll}
\rotate
\tablewidth{0pt}

\tabletypesize{\scriptsize}
\tablecaption{Hectochelle Field 1 Velocity Data}
\tablehead{
  \colhead{2massID} &  \colhead{RV F1\_E1} & \colhead{RV F1\_E2} & \colhead{R F1\_E1} &\colhead{R F1\_E2}  \\
    \colhead{}    &  \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & & \\

   }
\startdata
0533333-043918 & -6.9 $\pm$ 0.2  & -6.3 $\pm$ 0.2  & 41.8 & 37.1 \\ 
0533364-044949 & 21.2 $\pm$ 1.8  & 27.6 $\pm$ 1.8  & 9.3 & 8.5 \\ 
0533377-043349 & 26.3 $\pm$ 0.3  & 25.6 $\pm$ 0.4  & 28.2 & 27.4 \\ 
0533391-043807 & 27.5 $\pm$ 0.7  & 29.6 $\pm$ 0.8  & 10.5 & 9.3 \\ 
0533431-044714 & 25.0 $\pm$ 0.9  & 25.2 $\pm$ 0.7  & 9.0 & 10.6 \\ 
0533445-045930 & 12.4 $\pm$ 0.2  & 13.6 $\pm$ 0.2  & 45.8 & 47.2 \\ 
0533457-044124 & 18.1 $\pm$ 0.4  & 18.8 $\pm$ 0.4  & 21.8 & 20.4 \\ 
0533477-045208 & 29.8 $\pm$ 0.5  & 29.7 $\pm$ 0.5  & 19.8 & 20.7 \\ 
0533478-045503 & 25.2 $\pm$ 0.5  & 23.2 $\pm$ 0.4  & 21.4 & 23.5 \\ 
0533481-043927 & 21.8 $\pm$ 1.3  & 19.4 $\pm$ 1.2  & 18.1 & 18.9 \\ 
0533497-043329 & 48.0 $\pm$ 0.4  & 48.5 $\pm$ 0.3  & 18.6 & 19.6 \\ 
0533507-050039 & 28.5 $\pm$ 0.5  & 23.8 $\pm$ 1.0  & 17.3 & 13.2 \\ 
0533513-044822 & 31.3 $\pm$ 0.4  & 30.5 $\pm$ 0.4  & 22.4 & 21.8 \\ 
0533524-044400 & -5.0 $\pm$ 0.2  & -4.6 $\pm$ 0.2  & 48.7 & 51.5 \\ 
0533541-050340 & 24.9 $\pm$ 1.1  & 24.4 $\pm$ 0.8  & 9.3 & 12.5 \\ 
0533573-045915 & 21.9 $\pm$ 0.9  & 24.3 $\pm$ 0.8  & 9.5 & 10.3 \\ 
0534004-043615 & 39.1 $\pm$ 2.3  & 25.8 $\pm$ 2.2  & 9.4 & 8.6 \\ 
0534038-043606 & 31.7 $\pm$ 0.4  & 30.0 $\pm$ 0.4  & 21.5 & 24.3 \\ 
0534073-043231 & -12.9 $\pm$ 0.2  & -12.4 $\pm$ 0.2  & 42.6 & 48.1 \\ 
0534081-044357 & 21.4 $\pm$ 0.2  & 21.2 $\pm$ 0.3  & 30.8 & 27.8 \\ 
0534082-042600 & 30.3 $\pm$ 0.5  & 31.8 $\pm$ 0.6  & 19.7 & 16.1 \\ 
0534095-050111 & -7.3 $\pm$ 0.4  & -5.0 $\pm$ 0.4  & 16.3 & 18.1 \\ 
0534097-044846 & 21.1 $\pm$ 0.6  & 24.2 $\pm$ 0.8  & 14.2 & 12.7 \\ 
0534098-042819 & 53.9 $\pm$ 0.1  & 53.8 $\pm$ 0.1  & 54.4 & 53.0 \\ 
0534104-045035 & 24.9 $\pm$ 0.3  & 22.4 $\pm$ 0.3  & 40.2 & 37.8 \\ 
0534104-051020 & -42.5 $\pm$ 0.3  & -41.2 $\pm$ 0.2  & 22.4 & 29.7 \\ 
0534148-051418 & 26.4 $\pm$ 0.8  & 29.0 $\pm$ 0.6  & 10.5 & 15.9 \\ 
0534203-043403 & 23.8 $\pm$ 0.4  & 25.1 $\pm$ 0.5  & 20.6 & 17.2 \\ 
0534208-050650 & 27.8 $\pm$ 1.0  & 22.4 $\pm$ 0.9  & 6.5 & 9.2 \\ 
0534229-044139 & 30.1 $\pm$ 0.4  & 30.6 $\pm$ 0.4  & 25.8 & 25.6 \\ 
0534242-042439 & 9.3 $\pm$ 0.2  & 10.3 $\pm$ 0.2  & 53.8 & 53.2 \\ 
0534252-045439 & 21.9 $\pm$ 2.0  & 19.8 $\pm$ 1.3  & 7.4 & 10.4 \\ 
0534257-045655 & 25.2 $\pm$ 0.3  & 25.1 $\pm$ 0.4  & 28.1 & 27.8 \\ 
0534267-045045 & 35.0 $\pm$ 0.5  & 35.6 $\pm$ 0.5  & 18.9 & 21.2 \\ 
0534267-050117 & 30.9 $\pm$ 0.6  & 30.0 $\pm$ 0.5  & 16.6 & 21.4 \\ 
0534286-043439 & 16.9 $\pm$ 1.3  & 22.0 $\pm$ 1.2  & 15.4 & 16.0 \\ 
0534292-051439 & 29.2 $\pm$ 0.3  & 27.8 $\pm$ 0.3  & 36.6 & 34.4 \\ 
0534300-044950 & 27.5 $\pm$ 0.3  & 27.3 $\pm$ 0.3  & 28.9 & 29.2 \\ 
0534302-045830 & 20.7 $\pm$ 1.8  & 23.0 $\pm$ 1.5  & 13.5 & 15.5 \\ 
0534303-045705 & 26.7 $\pm$ 0.6  & 32.0 $\pm$ 0.7  & 14.3 & 13.7 \\ 
0534305-043351 & 18.3 $\pm$ 0.3  & 19.8 $\pm$ 0.3  & 21.4 & 21.7 \\ 
0534306-043552 & 28.2 $\pm$ 0.4  & 27.6 $\pm$ 0.6  & 22.2 & 14.8 \\ 
0534332-042713 & 19.6 $\pm$ 0.6  & 22.4 $\pm$ 0.6  & 13.4 & 13.3 \\ 
0534334-044332 & -48.0 $\pm$ 0.4  & -46.4 $\pm$ 0.4  & 22.3 & 20.6 \\ 
0534341-044827 & 25.5 $\pm$ 0.4  & 27.0 $\pm$ 0.4  & 20.7 & 20.4 \\ 
0534341-050517 & 34.7 $\pm$ 1.3  & 33.1 $\pm$ 0.8  & 7.0 & 13.1 \\ 
0534370-043310 & -0.6 $\pm$ 0.6  & 1.0 $\pm$ 0.5  & 11.8 & 15.1 \\ 
0534379-045108 & 32.0 $\pm$ 0.5  & 32.9 $\pm$ 0.5  & 19.8 & 20.0 \\ 
0534381-050457 & 57.5 $\pm$ 0.2  & 57.2 $\pm$ 0.1  & 44.5 & 54.7 \\ 
0534406-044331 & 27.3 $\pm$ 1.1  & 32.5 $\pm$ 0.8  & 7.1 & 10.5 \\ 
0534417-045346 & 31.7 $\pm$ 0.5  & 31.2 $\pm$ 0.4  & 19.2 & 22.6 \\ 
0534435-045136 & 28.4 $\pm$ 0.6  & 31.6 $\pm$ 0.5  & 12.2 & 14.9 \\ 
0534452-044758 & 33.5 $\pm$ 0.4  & 33.1 $\pm$ 0.3  & 17.3 & 24.8 \\ 
0534455-043607 & 32.4 $\pm$ 0.3  & 30.4 $\pm$ 0.3  & 36.3 & 37.3 \\ 
0534462-043009 & 4.0 $\pm$ 0.2  & 5.6 $\pm$ 0.2  & 38.9 & 38.9 \\ 
0534482-050713 & 20.8 $\pm$ 0.4  & 21.8 $\pm$ 0.3  & 21.3 & 27.3 \\ 
0534489-045714 & 30.6 $\pm$ 0.9  & 27.3 $\pm$ 0.6  & 8.1 & 13.0 \\ 
0534514-050011 & 28.8 $\pm$ 0.9  & 30.8 $\pm$ 0.6  & 8.6 & 14.2 \\ 
0534522-044011 & 68.3 $\pm$ 0.3  & 63.2 $\pm$ 0.3  & 36.3 & 37.3 \\ 
0534527-050050 & 24.4 $\pm$ 1.2  & 24.7 $\pm$ 0.8  & 9.2 & 12.5 \\ 
0534530-050327 & 24.2 $\pm$ 1.3  & 20.8 $\pm$ 2.1  & 6.5 & 3.7 \\ 
0534534-042909 & 31.5 $\pm$ 1.2  & 30.1 $\pm$ 1.8  & 6.3 & 8.2 \\ 
0534537-050548 & 24.2 $\pm$ 0.6  & 25.5 $\pm$ 0.6  & 12.3 & 13.8 \\ 
0534549-051702 & -64.7 $\pm$ 2.6  & 24.0 $\pm$ 0.7  & 3.5 & 11.2 \\ 
0534560-043812 & 30.6 $\pm$ 0.6  & 27.9 $\pm$ 0.5  & 16.3 & 18.7 \\ 
0534561-050601 & 32.8 $\pm$ 1.3  & 28.9 $\pm$ 1.4  & 11.2 & 12.7 \\ 
0534568-044604 & 30.7 $\pm$ 0.4  & 30.1 $\pm$ 0.3  & 26.6 & 31.1 \\ 
0534581-043718 & 29.3 $\pm$ 0.6  & 30.8 $\pm$ 0.5  & 14.8 & 18.8 \\ 
0535009-044819 & 30.9 $\pm$ 0.7  & 29.4 $\pm$ 0.6  & 12.1 & 16.6 \\ 
0535016-043252 & 29.0 $\pm$ 0.4  & 27.6 $\pm$ 0.4  & 24.6 & 24.3 \\ 
0535020-051537 & 29.6 $\pm$ 0.6  & 26.2 $\pm$ 0.4  & 14.8 & 22.1 \\ 
0535050-043233 & 33.5 $\pm$ 1.0  & 38.2 $\pm$ 1.3  & 9.3 & 9.2 \\ 
0535050-043733 & -3.3 $\pm$ 0.5  & -4.4 $\pm$ 0.5  & 20.0 & 19.1 \\ 
0535052-051450 & 19.5 $\pm$ 0.3  & 22.2 $\pm$ 0.3  & 38.6 & 39.5 \\ 
0535054-042506 & 28.9 $\pm$ 0.3  & 29.3 $\pm$ 0.3  & 26.9 & 28.3 \\ 
0535075-051114 & 20.4 $\pm$ 0.8  & 16.8 $\pm$ 1.9  & 11.4 & 4.0 \\ 
0535096-043311 & 4.5 $\pm$ 0.4  & 5.6 $\pm$ 0.4  & 21.5 & 22.8 \\ 
0535115-044633 & 22.0 $\pm$ 0.7  & 22.2 $\pm$ 0.6  & 18.9 & 20.0 \\ 
0535122-042711 & 28.4 $\pm$ 0.4  & 27.9 $\pm$ 0.4  & 24.1 & 23.3 \\ 
0535132-044154 & 29.2 $\pm$ 0.7  & 31.5 $\pm$ 0.6  & 12.3 & 16.2 \\ 
0535146-050852 & 27.5 $\pm$ 1.3  & 28.4 $\pm$ 1.6  & 8.9 & 10.0 \\ 
0535153-043326 & 28.8 $\pm$ 0.3  & 29.0 $\pm$ 0.3  & 34.8 & 33.9 \\ 
0535164-045802 & 24.3 $\pm$ 0.8  & 23.7 $\pm$ 1.0  & 11.2 & 9.4 \\ 
0535178-044452 & 30.3 $\pm$ 0.3  & 28.8 $\pm$ 0.5  & 33.6 & 20.8 \\ 
0535179-051532 & 29.8 $\pm$ 1.0  & 29.0 $\pm$ 1.0  & 11.9 & 11.3 \\ 
0535180-043119 & 28.8 $\pm$ 2.6  & 31.9 $\pm$ 2.5  & 9.2 & 10.0 \\ 
0535201-044134 & 29.5 $\pm$ 1.5  & 30.9 $\pm$ 0.7  & 6.1 & 12.2 \\ 
0535203-050226 & 30.2 $\pm$ 0.7  & 28.3 $\pm$ 0.6  & 13.2 & 15.7 \\ 
0535210-044538 & 33.9 $\pm$ 0.8  & 30.5 $\pm$ 0.8  & 11.5 & 11.3 \\ 
0535228-043740 & 26.8 $\pm$ 2.0  & 26.3 $\pm$ 0.8  & 4.2 & 10.3 \\ 
0535228-044641 & 31.8 $\pm$ 0.7  & 30.8 $\pm$ 0.4  & 16.2 & 22.7 \\ 
0535241-045008 & 32.3 $\pm$ 0.7  & 30.4 $\pm$ 0.7  & 12.6 & 13.1 \\ 
0535256-045718 & 26.7 $\pm$ 2.6  & 20.6 $\pm$ 0.8  & 6.5 & 12.2 \\ 
0535265-045606 & 29.0 $\pm$ 1.3  & 30.2 $\pm$ 1.3  & 18.1 & 17.3 \\ 
0535268-051107 & 28.9 $\pm$ 0.4  & 33.5 $\pm$ 0.4  & 30.2 & 28.6 \\ 
0535274-051709 & 26.7 $\pm$ 0.8  & 26.5 $\pm$ 0.6  & 11.8 & 15.4 \\ 
0535286-044726 & 25.1 $\pm$ 1.3  & 26.2 $\pm$ 0.9  & 5.8 & 8.4 \\ 
0535294-043820 & 40.9 $\pm$ 6.7  & 34.5 $\pm$ 2.4  & 4.5 & 6.0 \\ 
0535298-051210 & 60.9 $\pm$ 1.2  & 35.5 $\pm$ 2.4  & 7.1 & 10.6 \\ 
0535299-044951 & 29.4 $\pm$ 0.4  & 28.9 $\pm$ 0.4  & 28.5 & 28.1 \\ 
0535305-045128 & 28.7 $\pm$ 0.3  & 29.0 $\pm$ 0.3  & 32.5 & 31.8 \\ 
0535306-043900 & 32.7 $\pm$ 0.9  & 30.3 $\pm$ 0.6  & 10.8 & 14.7 \\ 
0535319-050928 & 29.8 $\pm$ 0.4  & 30.3 $\pm$ 0.3  & 28.4 & 30.1 \\ 
0535333-045111 & 29.7 $\pm$ 0.7  & 28.8 $\pm$ 0.5  & 13.0 & 18.7 \\ 
0535334-045601 & 33.7 $\pm$ 4.7  & 31.9 $\pm$ 1.7  & 6.0 & 10.8 \\ 
0535340-043237 & 33.4 $\pm$ 1.7  & 32.5 $\pm$ 1.8  & 10.4 & 9.5 \\ 
0535340-045411 & 30.1 $\pm$ 0.5  & 30.4 $\pm$ 0.4  & 19.1 & 23.3 \\ 
0535344-044020 & 30.7 $\pm$ 0.4  & 29.5 $\pm$ 0.4  & 23.5 & 23.0 \\ 
0535352-044739 & 31.3 $\pm$ 0.3  & 30.2 $\pm$ 0.4  & 27.3 & 25.6 \\ 
0535366-050414 & 25.7 $\pm$ 0.4  & 27.1 $\pm$ 0.4  & 22.5 & 23.8 \\ 
0535379-045229 & -3.1 $\pm$ 3.2  & 10.7 $\pm$ 1.3  & 3.7 & 5.5 \\ 
0535380-044833 & 31.3 $\pm$ 0.4  & 31.7 $\pm$ 0.4  & 24.8 & 25.3 \\ 
0535385-045941 & 32.1 $\pm$ 2.6  & 25.6 $\pm$ 0.8  & 3.9 & 10.8 \\ 
0535394-044019 & 30.9 $\pm$ 0.7  & 31.9 $\pm$ 0.8  & 21.5 & 19.1 \\ 
0535398-044404 & 31.9 $\pm$ 0.4  & 30.7 $\pm$ 0.4  & 25.1 & 26.6 \\ 
0535400-044555 & 29.1 $\pm$ 0.4  & 29.3 $\pm$ 0.3  & 27.3 & 28.9 \\ 
0535430-050307 & 19.4 $\pm$ 0.9  & 19.4 $\pm$ 0.9  & 8.0 & 8.1 \\ 
0535449-043054 & 22.3 $\pm$ 0.5  & 20.0 $\pm$ 0.5  & 16.4 & 14.2 \\ 
0535450-045141 & 10.7 $\pm$ 4.3  & 27.3 $\pm$ 2.0  & 7.5 & 9.4 \\ 
0535453-044339 & 25.3 $\pm$ 0.6  & 25.5 $\pm$ 0.5  & 21.8 & 25.0 \\ 
0535474-051028 & 21.8 $\pm$ 1.7  & 26.1 $\pm$ 1.3  & 4.8 & 7.0 \\ 
0535488-050028 & 23.1 $\pm$ 2.7  & 26.1 $\pm$ 2.0  & 10.0 & 13.3 \\ 
0535489-050139 & 27.8 $\pm$ 0.5  & 26.7 $\pm$ 0.4  & 21.5 & 24.5 \\ 
0535491-045306 & 46.6 $\pm$ 3.0  & 8.8 $\pm$ 1.8  & 3.5 & 4.3 \\ 
0535495-042438 & 24.5 $\pm$ 1.0  & 26.3 $\pm$ 1.0  & 20.9 & 20.1 \\ 
0535498-044632 & 31.2 $\pm$ 1.5  & 29.1 $\pm$ 1.2  & 5.2 & 5.6 \\ 
0535503-044208 & 38.4 $\pm$ 3.1  & 91.5 $\pm$ 1.6  & 4.6 & 5.1 \\ 
0535511-050708 & 27.8 $\pm$ 0.4  & 24.2 $\pm$ 0.4  & 25.5 & 25.1 \\ 
0535518-045410 & 24.1 $\pm$ 0.2  & 24.6 $\pm$ 0.2  & 49.9 & 49.6 \\ 
0535535-050234 & 26.3 $\pm$ 1.1  & 32.1 $\pm$ 0.8  & 8.5 & 11.7 \\ 
0535540-044719 & 25.3 $\pm$ 1.7  & 26.4 $\pm$ 0.9  & 3.8 & 9.6 \\ 
0535540-050414 & 24.7 $\pm$ 0.5  & 27.2 $\pm$ 0.4  & 20.9 & 24.7 \\ 
0535560-045655 & 27.3 $\pm$ 0.3  & 28.1 $\pm$ 0.3  & 35.1 & 36.1 \\ 
0535572-043203 & 1.9 $\pm$ 0.2  & 2.6 $\pm$ 0.2  & 41.5 & 41.0 \\ 
0535586-042924 & 34.9 $\pm$ 1.0  & 35.9 $\pm$ 0.8  & 7.1 & 10.3 \\ 
0535592-045846 & 28.5 $\pm$ 0.4  & 29.3 $\pm$ 0.4  & 26.6 & 25.2 \\ 
0536002-044346 & 29.0 $\pm$ 0.4  & 27.9 $\pm$ 0.4  & 22.5 & 23.4 \\ 
0536008-044258 & -165.1 $\pm$ 1.7  & 28.9 $\pm$ 1.5  & 3.6 & 5.1 \\ 
0536017-043417 & 27.6 $\pm$ 0.3  & 26.9 $\pm$ 0.3  & 30.3 & 29.7 \\ 
0536033-045740 & 24.3 $\pm$ 0.8  & 24.1 $\pm$ 0.7  & 15.6 & 17.5 \\ 
0536051-045103 & 29.0 $\pm$ 0.7  & 28.1 $\pm$ 0.5  & 17.7 & 22.6 \\ 
0536068-050615 & 21.5 $\pm$ 0.5  & 20.8 $\pm$ 0.4  & 18.8 & 23.0 \\ 
0536080-044120 & 25.1 $\pm$ 0.8  & 27.0 $\pm$ 0.5  & 11.4 & 18.5 \\ 
0536092-045000 & 21.3 $\pm$ 1.2  & 21.7 $\pm$ 0.7  & 7.8 & 14.2 \\ 
0536118-051555 & 23.3 $\pm$ 0.7  & 24.8 $\pm$ 0.6  & 11.8 & 14.0 \\ 
0536163-044642 & -17.6 $\pm$ 0.2  & -16.7 $\pm$ 0.2  & 41.9 & 49.4 \\ 
0536164-045758 & 47.0 $\pm$ 0.7  & 47.9 $\pm$ 0.6  & 10.4 & 13.4 \\ 
0536191-042730 & 29.5 $\pm$ 0.4  & 29.2 $\pm$ 0.4  & 22.3 & 23.9 \\ 
0536197-044455 & 29.9 $\pm$ 0.3  & 30.3 $\pm$ 0.3  & 34.3 & 33.5 \\ 
0536285-043359 & 67.3 $\pm$ 0.8  & 77.9 $\pm$ 2.0  & 7.1 & 5.2 \\ 
0536292-045351 & 26.2 $\pm$ 0.5  & 27.6 $\pm$ 0.5  & 18.8 & 17.9 \\ 
0536295-043957 & -13.9 $\pm$ 0.2  & -12.7 $\pm$ 0.2  & 37.3 & 37.8 \\ 
0536398-043751 & 22.1 $\pm$ 0.3  & 22.2 $\pm$ 0.3  & 28.6 & 31.2 \\ 
0536493-044905 & -8.7 $\pm$ 0.2  & -7.8 $\pm$ 0.3  & 35.2 & 32.3 \\ 
0536494-045748 & 19.5 $\pm$ 0.4  & 20.8 $\pm$ 0.3  & 20.2 & 25.6 \\ 
0537086-044942 & 41.5 $\pm$ 0.2  & 41.4 $\pm$ 0.2  & 36.1 & 38.4 \\ 
\enddata
\end{deluxetable}


==> tab5-full.tex <==
\begin{deluxetable}{lllll}
\rotate
\tablewidth{0pt}

\tabletypesize{\scriptsize}
\tablecaption{Hectochelle Field 2 Velocity Data}
\tablehead{
  \colhead{2massID} &  \colhead{RV F2\_E1} & \colhead{RV F2\_E2} & \colhead{R F2\_E1} &\colhead{R F2\_E2}  \\
    \colhead{}    &  \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & & \\

   }
\startdata
0533233-052153 & 47.2 $\pm$ 0.4  & 47.2 $\pm$ 0.4  & 20.1 & 24.1 \\ 
0533263-051640 & 67.6 $\pm$ 0.6  & 49.5 $\pm$ 2.5  & 12.1 & 9.4 \\ 
0533289-050930 & 106.8 $\pm$ 0.3  & 106.3 $\pm$ 0.2  & 31.4 & 39.6 \\ 
0533293-050749 & 32.6 $\pm$ 0.8  & 31.4 $\pm$ 0.8  & 11.8 & 13.3 \\ 
0533357-050923 & 30.6 $\pm$ 3.4  & 31.0 $\pm$ 2.5  & 9.3 & 10.6 \\ 
0533406-050046 & 28.4 $\pm$ 0.5  & -76.7 $\pm$ 2.0  & 19.6 & 4.0 \\ 
0533435-053225 & 54.2 $\pm$ 0.4  & 53.4 $\pm$ 0.3  & 16.0 & 22.6 \\ 
0533482-053447 & 21.8 $\pm$ 1.0  & 27.7 $\pm$ 1.1  & 7.5 & 8.7 \\ 
0533483-052239 & 25.3 $\pm$ 0.4  & 25.5 $\pm$ 0.3  & 23.4 & 26.7 \\ 
0533489-051753 & 25.2 $\pm$ 0.6  & 24.6 $\pm$ 0.4  & 14.7 & 26.5 \\ 
0533520-050655 & -8.6 $\pm$ 0.5  & -9.7 $\pm$ 0.7  & 14.7 & 11.2 \\ 
0533565-050647 & 31.4 $\pm$ 0.4  & 30.6 $\pm$ 0.4  & 26.8 & 29.5 \\ 
0534037-052218 & 20.3 $\pm$ 0.4  & 19.3 $\pm$ 0.6  & 19.6 & 13.8 \\ 
0534095-050111 & -5.5 $\pm$ 0.5  & -2.1 $\pm$ 0.5  & 13.3 & 15.6 \\ 
0534120-052419 & 19.2 $\pm$ 1.5  & 19.1 $\pm$ 0.8  & 5.1 & 10.8 \\ 
0534141-053653 & 26.0 $\pm$ 0.5  & 26.9 $\pm$ 0.5  & 36.3 & 36.6 \\ 
0534164-053645 & 26.9 $\pm$ 0.2  & 26.9 $\pm$ 0.2  & 37.5 & 40.6 \\ 
0534168-050421 & 31.7 $\pm$ 0.4  & 31.7 $\pm$ 0.4  & 27.6 & 27.9 \\ 
0534172-052904 & -51.4 $\pm$ 1.1  & 25.1 $\pm$ 1.0  & 4.4 & 9.0 \\ 
0534174-053158 & 26.0 $\pm$ 0.4  & 26.4 $\pm$ 0.3  & 21.9 & 28.9 \\ 
0534196-050229 & 41.7 $\pm$ 0.8  & 31.8 $\pm$ 0.7  & 9.6 & 12.9 \\ 
0534203-045856 & 27.7 $\pm$ 0.5  & 27.6 $\pm$ 0.4  & 16.4 & 19.7 \\ 
0534214-045547 & 21.2 $\pm$ 1.3  & 20.0 $\pm$ 0.8  & 6.5 & 10.2 \\ 
0534215-051013 & 109.0 $\pm$ 0.9  & 8.7 $\pm$ 0.7  & 6.7 & 10.4 \\ 
0534238-050815 & 25.1 $\pm$ 0.9  & 27.3 $\pm$ 0.6  & 12.8 & 16.4 \\ 
0534254-045655 & 26.5 $\pm$ 0.6  & 24.2 $\pm$ 0.6  & 15.9 & 14.0 \\ 
0534261-052630 & 30.9 $\pm$ 1.4  & 24.7 $\pm$ 1.2  & 4.5 & 7.2 \\ 
0534265-052323 & 26.2 $\pm$ 1.0  & 25.6 $\pm$ 0.9  & 8.6 & 10.1 \\ 
0534267-054157 & 26.1 $\pm$ 1.0  & 27.4 $\pm$ 0.5  & 7.4 & 15.1 \\ 
0534278-054331 & 27.6 $\pm$ 1.7  & 21.2 $\pm$ 1.3  & 6.2 & 9.7 \\ 
0534298-050405 & 27.8 $\pm$ 0.5  & 27.0 $\pm$ 0.4  & 19.9 & 20.3 \\ 
0534316-052826 & 23.7 $\pm$ 0.9  & 25.0 $\pm$ 0.5  & 10.8 & 19.3 \\ 
0534338-052718 & 22.9 $\pm$ 1.3  & 21.2 $\pm$ 0.9  & 4.5 & 9.0 \\ 
0534339-053451 & 30.2 $\pm$ 0.8  & 26.7 $\pm$ 0.5  & 13.3 & 23.8 \\ 
0534356-052952 & 18.0 $\pm$ 0.8  & 20.6 $\pm$ 0.6  & 9.3 & 13.5 \\ 
0534359-051524 & 24.4 $\pm$ 0.4  & 24.6 $\pm$ 0.4  & 19.9 & 22.5 \\ 
0534375-054117 & 34.5 $\pm$ 1.4  & 28.7 $\pm$ 0.6  & 11.5 & 20.9 \\ 
0534375-054310 & 24.7 $\pm$ 0.7  & 27.8 $\pm$ 0.4  & 10.9 & 22.1 \\ 
0534390-045528 & 56.1 $\pm$ 0.6  & 48.1 $\pm$ 0.6  & 15.2 & 14.8 \\ 
0534404-045739 & 26.7 $\pm$ 1.3  & 28.2 $\pm$ 0.7  & 6.0 & 12.0 \\ 
0534427-052837 & 23.0 $\pm$ 0.7  & 21.9 $\pm$ 0.4  & 12.6 & 21.4 \\ 
0534428-052516 & 34.3 $\pm$ 1.0  & 31.0 $\pm$ 0.5  & 7.3 & 17.3 \\ 
0534449-050649 & 30.2 $\pm$ 0.4  & 30.1 $\pm$ 0.3  & 29.8 & 33.0 \\ 
0534454-050207 & 29.2 $\pm$ 0.3  & 29.0 $\pm$ 0.3  & 26.5 & 29.2 \\ 
0534479-050455 & 30.0 $\pm$ 0.4  & 29.2 $\pm$ 0.3  & 24.1 & 27.3 \\ 
0534487-051746 & 23.5 $\pm$ 1.6  & 21.2 $\pm$ 0.8  & 4.6 & 10.5 \\ 
0534487-051907 & 17.3 $\pm$ 3.5  & 20.9 $\pm$ 0.8  & 6.8 & 12.1 \\ 
0534499-051844 & 55.6 $\pm$ 5.4  & 58.8 $\pm$ 5.4  & 7.0 & 7.3 \\ 
0534534-051027 & 23.2 $\pm$ 0.5  & 23.1 $\pm$ 0.4  & 16.0 & 19.1 \\ 
0534543-051721 & 29.0 $\pm$ 1.9  & 26.3 $\pm$ 1.1  & 5.3 & 9.0 \\ 
0534545-045605 & 26.8 $\pm$ 1.7  & 32.7 $\pm$ 1.5  & 6.5 & 7.3 \\ 
0534556-052937 & 20.5 $\pm$ 1.2  & 19.6 $\pm$ 0.7  & 5.9 & 11.7 \\ 
0534572-054202 & 23.4 $\pm$ 1.0  & 27.4 $\pm$ 0.6  & 7.6 & 14.5 \\ 
0534590-054429 & 19.4 $\pm$ 1.1  & 23.3 $\pm$ 0.9  & 10.0 & 10.7 \\ 
0534593-050530 & 29.6 $\pm$ 0.5  & 26.1 $\pm$ 0.4  & 16.9 & 21.9 \\ 
0535012-052016 & 28.3 $\pm$ 0.7  & 27.9 $\pm$ 0.6  & 11.8 & 15.4 \\ 
0535024-052046 & 24.9 $\pm$ 0.4  & 25.1 $\pm$ 0.3  & 24.3 & 30.3 \\ 
0535030-045959 & 25.8 $\pm$ 1.9  & 26.6 $\pm$ 1.8  & 8.2 & 9.9 \\ 
0535033-045643 & 26.4 $\pm$ 0.5  & 26.4 $\pm$ 0.6  & 22.1 & 19.0 \\ 
0535039-052903 & 11.2 $\pm$ 0.8  & 48.8 $\pm$ 0.7  & 17.5 & 15.5 \\ 
0535047-052638 & 25.5 $\pm$ 0.8  & 26.5 $\pm$ 0.8  & 12.3 & 11.0 \\ 
0535053-053428 & 23.6 $\pm$ 0.4  & 25.6 $\pm$ 0.4  & 26.1 & 28.7 \\ 
0535056-052519 & 25.6 $\pm$ 0.7  & 29.1 $\pm$ 0.8  & 15.0 & 13.8 \\ 
0535068-051038 & 27.7 $\pm$ 2.5  & 20.0 $\pm$ 0.9  & 4.9 & 11.4 \\ 
0535080-053244 & 28.5 $\pm$ 0.8  & 29.0 $\pm$ 0.6  & 11.6 & 15.8 \\ 
0535087-050440 & 31.5 $\pm$ 1.4  & 25.4 $\pm$ 1.0  & 7.0 & 10.3 \\ 
0535103-054633 & 17.8 $\pm$ 0.2  & 19.1 $\pm$ 0.2  & 40.5 & 44.0 \\ 
0535121-053138 & 33.6 $\pm$ 3.9  & 33.1 $\pm$ 1.8  & 7.6 & 7.0 \\ 
0535125-052344 & 26.3 $\pm$ 0.5  & 23.8 $\pm$ 0.7  & 26.4 & 21.9 \\ 
0535143-045522 & 22.4 $\pm$ 1.3  & 23.7 $\pm$ 1.1  & 6.5 & 8.8 \\ 
0535146-050852 & 22.6 $\pm$ 1.5  & 29.6 $\pm$ 1.2  & 8.6 & 10.3 \\ 
0535149-053639 & 27.9 $\pm$ 1.0  & 27.8 $\pm$ 0.8  & 9.6 & 11.4 \\ 
0535152-050033 & 31.0 $\pm$ 1.4  & 34.3 $\pm$ 1.4  & 5.1 & 5.2 \\ 
0535153-051902 & -59.4 $\pm$ 4.0  & -63.0 $\pm$ 3.0  & 4.0 & 3.7 \\ 
0535156-052403 & -13.1 $\pm$ 0.7  & -9.4 $\pm$ 0.8  & 14.8 & 13.1 \\ 
0535159-051459 & 26.5 $\pm$ 0.3  & 26.5 $\pm$ 0.3  & 31.9 & 32.7 \\ 
0535210-052809 & 29.3 $\pm$ 0.7  & 30.1 $\pm$ 0.7  & 14.8 & 13.9 \\ 
0535211-051821 & 27.0 $\pm$ 1.6  & 23.7 $\pm$ 0.9  & 5.7 & 9.7 \\ 
0535213-052345 & 25.7 $\pm$ 1.1  & 22.7 $\pm$ 1.7  & 7.8 & 4.7 \\ 
0535216-052526 & 22.3 $\pm$ 0.9  & 22.8 $\pm$ 1.1  & 10.2 & 7.2 \\ 
0535216-053458 & 25.2 $\pm$ 0.7  & 25.3 $\pm$ 0.8  & 13.4 & 12.6 \\ 
0535219-051704 & 29.1 $\pm$ 1.6  & 29.3 $\pm$ 1.4  & 4.5 & 5.6 \\ 
0535223-050804 & 30.8 $\pm$ 1.0  & 29.8 $\pm$ 1.0  & 8.2 & 9.3 \\ 
0535228-054442 & 19.7 $\pm$ 7.2  & 27.5 $\pm$ 7.5  & 4.4 & 5.0 \\ 
0535252-050927 & 26.8 $\pm$ 0.4  & 28.8 $\pm$ 0.5  & 21.4 & 20.8 \\ 
0535254-052135 & 31.3 $\pm$ 1.3  & 28.5 $\pm$ 1.6  & 6.5 & 5.3 \\ 
0535256-050757 & 29.3 $\pm$ 0.9  & 26.6 $\pm$ 0.8  & 10.6 & 12.4 \\ 
0535256-053020 & 26.3 $\pm$ 0.3  & 26.7 $\pm$ 0.4  & 29.8 & 28.4 \\ 
0535262-052006 & 31.5 $\pm$ 1.2  & 27.2 $\pm$ 0.6  & 7.2 & 15.4 \\ 
0535265-045606 & 30.4 $\pm$ 1.3  & 31.7 $\pm$ 1.2  & 18.8 & 19.8 \\ 
0535279-051657 & 30.1 $\pm$ 0.6  & 28.8 $\pm$ 0.6  & 17.0 & 19.6 \\ 
0535289-051618 & 32.4 $\pm$ 0.7  & 30.9 $\pm$ 1.4  & 13.6 & 6.4 \\ 
0535304-052538 & 20.4 $\pm$ 1.9  & 22.5 $\pm$ 1.4  & 4.4 & 5.7 \\ 
0535306-052716 & 18.7 $\pm$ 1.5  & 15.3 $\pm$ 2.0  & 4.8 & 4.0 \\ 
0535308-045517 & 23.3 $\pm$ 1.2  & 25.5 $\pm$ 0.6  & 6.9 & 15.2 \\ 
0535309-051817 & 25.2 $\pm$ 1.2  & 24.5 $\pm$ 1.2  & 14.6 & 13.2 \\ 
0535313-053308 & 26.6 $\pm$ 0.8  & 26.2 $\pm$ 0.8  & 24.0 & 24.0 \\ 
0535351-052123 & 20.3 $\pm$ 1.4  & 23.5 $\pm$ 1.0  & 6.3 & 7.0 \\ 
0535353-051111 & 26.6 $\pm$ 0.6  & 27.1 $\pm$ 0.6  & 15.2 & 13.5 \\ 
0535364-050115 & 28.2 $\pm$ 0.3  & 26.4 $\pm$ 0.3  & 40.5 & 36.0 \\ 
0535364-053411 & 25.6 $\pm$ 0.5  & 26.0 $\pm$ 0.6  & 17.2 & 17.4 \\ 
0535382-051419 & 29.1 $\pm$ 1.6  & 29.6 $\pm$ 1.5  & 12.0 & 12.4 \\ 
0535419-052812 & 25.6 $\pm$ 0.5  & 24.5 $\pm$ 0.5  & 32.3 & 30.9 \\ 
0535420-051259 & 35.2 $\pm$ 1.5  & 29.2 $\pm$ 0.9  & 4.3 & 8.2 \\ 
0535433-053244 & 30.8 $\pm$ 0.7  & 30.7 $\pm$ 0.6  & 15.1 & 17.7 \\ 
0535435-050541 & 26.5 $\pm$ 0.9  & 27.2 $\pm$ 0.6  & 9.2 & 14.9 \\ 
0535454-052036 & 24.1 $\pm$ 1.7  & 26.4 $\pm$ 1.4  & 15.5 & 17.8 \\ 
0535474-052249 & 28.6 $\pm$ 0.4  & 28.1 $\pm$ 0.4  & 25.7 & 27.0 \\ 
0535476-051914 & 21.1 $\pm$ 1.4  & 21.4 $\pm$ 1.2  & 5.0 & 6.2 \\ 
0535488-050028 & 25.0 $\pm$ 3.1  & 19.1 $\pm$ 2.2  & 8.7 & 11.0 \\ 
0535504-052835 & 45.1 $\pm$ 4.0  & 56.8 $\pm$ 2.6  & 9.2 & 10.1 \\ 
0535510-051509 & 27.9 $\pm$ 0.4  & 28.3 $\pm$ 0.4  & 27.9 & 27.7 \\ 
0535546-050627 & 25.7 $\pm$ 1.3  & 21.7 $\pm$ 1.3  & 4.8 & 5.4 \\ 
0535546-052707 & 27.4 $\pm$ 0.4  & 28.6 $\pm$ 0.4  & 23.7 & 25.4 \\ 
0535547-051055 & 40.6 $\pm$ 0.2  & 40.6 $\pm$ 0.2  & 30.1 & 39.1 \\ 
0535549-051315 & 66.5 $\pm$ 0.2  & 66.4 $\pm$ 0.2  & 33.2 & 31.6 \\ 
0535575-053951 & 72.7 $\pm$ 3.5  & 65.1 $\pm$ 2.6  & 6.3 & 9.2 \\ 
0536033-045740 & 23.3 $\pm$ 1.1  & 26.2 $\pm$ 0.8  & 11.4 & 13.2 \\ 
0536073-054221 & 22.7 $\pm$ 0.3  & 23.7 $\pm$ 0.3  & 33.0 & 33.6 \\ 
0536118-050032 & 26.6 $\pm$ 0.3  & 26.5 $\pm$ 0.4  & 26.0 & 25.8 \\ 
0536169-051142 & 25.6 $\pm$ 0.3  & 24.4 $\pm$ 0.3  & 34.6 & 33.7 \\ 
0536187-051218 & 22.5 $\pm$ 0.8  & 23.1 $\pm$ 0.6  & 10.8 & 15.1 \\ 
0536262-051653 & 26.8 $\pm$ 1.0  & 25.6 $\pm$ 0.9  & 8.6 & 7.4 \\ 
0536283-052142 & 9.5 $\pm$ 2.3  & -0.7 $\pm$ 1.4  & 4.0 & 4.2 \\ 
0536340-053405 & 20.1 $\pm$ 3.4  & 32.5 $\pm$ 2.8  & 5.2 & 8.7 \\ 
0536360-051135 & 21.0 $\pm$ 0.3  & 21.1 $\pm$ 0.3  & 26.1 & 35.6 \\ 
0536363-053634 & 36.4 $\pm$ 2.2  & 24.1 $\pm$ 1.3  & 8.5 & 14.9 \\ 
0536394-051919 & 54.8 $\pm$ 0.7  & 54.0 $\pm$ 0.5  & 17.2 & 19.0 \\ 
0536399-052123 & 26.1 $\pm$ 0.4  & 28.6 $\pm$ 0.4  & 23.4 & 22.1 \\ 
0536476-052050 & 33.1 $\pm$ 1.1  & 36.2 $\pm$ 0.9  & 8.1 & 10.4 \\ 
0536496-050409 & 21.1 $\pm$ 0.4  & 22.1 $\pm$ 0.4  & 21.0 & 23.5 \\ 
0536572-050604 & 27.2 $\pm$ 0.3  & 28.3 $\pm$ 0.3  & 31.1 & 29.2 \\ 
0537001-051411 & 34.4 $\pm$ 0.4  & 41.5 $\pm$ 0.5  & 18.7 & 15.6 \\ 
0537040-051901 & -31.3 $\pm$ 0.2  & -29.9 $\pm$ 0.2  & 36.3 & 35.7 \\ 
0537090-051712 & 39.1 $\pm$ 3.2  & 57.8 $\pm$ 1.3  & 7.3 & 7.4 \\ 
\enddata
\end{deluxetable}


==> tab6-full.tex <==
\begin{deluxetable}{lll}
\rotate
\tablewidth{0pt}

\tabletypesize{\scriptsize}
\tablecaption{Hectochelle Field 3 Velocity Data}
\tablehead{
  \colhead{2massID} &  \colhead{RV F3\_E1}  & \colhead{R F1\_E1}   \\
    \colhead{}    &  \colhead{(km s$^{-1}$)} &  \\

   }
\startdata
0533225-053240 & 24.7 $\pm$ 0.9  & 8.2  \\ 
0533256-052354 & 70.3 $\pm$ 0.4  & 22.8  \\ 
0533287-052610 & 30.4 $\pm$ 1.6  & 5.6  \\ 
0533298-052735 & -17.5 $\pm$ 0.5  & 18.3  \\ 
0533301-052257 & 22.6 $\pm$ 0.6  & 12.6  \\ 
0533307-050813 & -17.8 $\pm$ 0.8  & 5.5  \\ 
0533339-053326 & 29.6 $\pm$ 0.5  & 18.0  \\ 
0533344-051417 & 28.8 $\pm$ 0.8  & 11.2  \\ 
0533364-051153 & 20.7 $\pm$ 0.5  & 18.3  \\ 
0533385-051312 & 25.4 $\pm$ 1.1  & 7.0  \\ 
0533415-050934 & -12.7 $\pm$ 0.5  & 10.5  \\ 
0533416-052404 & 22.4 $\pm$ 0.4  & 19.9  \\ 
0533476-052548 & 28.6 $\pm$ 0.8  & 10.3  \\ 
0533545-051415 & 62.2 $\pm$ 0.5  & 14.7  \\ 
0533567-052133 & 24.5 $\pm$ 0.6  & 14.7  \\ 
0533570-054210 & 111.9 $\pm$ 0.9  & 7.1  \\ 
0533579-053626 & 29.1 $\pm$ 2.1  & 7.5  \\ 
0534022-053619 & 27.0 $\pm$ 0.5  & 24.2  \\ 
0534030-053657 & 27.1 $\pm$ 0.5  & 22.8  \\ 
0534059-052238 & 19.7 $\pm$ 1.1  & 7.8  \\ 
0534071-054925 & 47.4 $\pm$ 0.7  & 7.0  \\ 
0534074-051336 & 30.5 $\pm$ 0.5  & 17.6  \\ 
0534140-054721 & 30.5 $\pm$ 1.0  & 7.5  \\ 
0534142-054221 & 28.8 $\pm$ 0.7  & 15.1  \\ 
0534148-051418 & 28.0 $\pm$ 1.2  & 7.7  \\ 
0534156-053224 & 15.2 $\pm$ 1.3  & 6.2  \\ 
0534181-052833 & 13.4 $\pm$ 1.0  & 6.7  \\ 
0534185-050448 & 25.0 $\pm$ 0.5  & 30.1  \\ 
0534193-055026 & 31.8 $\pm$ 1.6  & 3.6  \\ 
0534195-053019 & 24.5 $\pm$ 0.5  & 30.9  \\ 
0534196-050229 & 50.8 $\pm$ 0.8  & 5.4  \\ 
0534207-053235 & 23.7 $\pm$ 1.1  & 9.7  \\ 
0534209-052448 & 29.5 $\pm$ 1.0  & 9.6  \\ 
0534212-053534 & 17.9 $\pm$ 0.9  & 7.8  \\ 
0534223-052226 & 13.7 $\pm$ 1.2  & 5.3  \\ 
0534260-050733 & 30.0 $\pm$ 1.7  & 4.2  \\ 
0534267-050117 & 34.5 $\pm$ 1.5  & 6.7  \\ 
0534275-052828 & 25.0 $\pm$ 0.8  & 12.4  \\ 
0534276-053719 & 19.3 $\pm$ 1.7  & 4.2  \\ 
0534278-054331 & 17.6 $\pm$ 1.1  & 9.8  \\ 
0534279-052634 & 24.6 $\pm$ 1.6  & 5.0  \\ 
0534301-054015 & 38.5 $\pm$ 1.5  & 4.9  \\ 
0534302-045830 & 61.5 $\pm$ 1.3  & 5.8  \\ 
0534311-052155 & 23.5 $\pm$ 1.0  & 9.2  \\ 
0534312-052854 & 24.4 $\pm$ 0.6  & 15.6  \\ 
0534320-052742 & 19.6 $\pm$ 1.4  & 5.3  \\ 
0534341-050517 & 34.1 $\pm$ 1.7  & 3.5  \\ 
0534357-054009 & 22.9 $\pm$ 0.9  & 10.0  \\ 
0534358-053645 & 28.3 $\pm$ 1.0  & 6.5  \\ 
0534360-054215 & 26.9 $\pm$ 0.4  & 26.0  \\ 
0534400-052604 & 14.9 $\pm$ 1.1  & 7.8  \\ 
0534408-052638 & 21.7 $\pm$ 1.0  & 8.4  \\ 
0534411-054739 & 17.0 $\pm$ 1.0  & 7.5  \\ 
0534412-054611 & 19.9 $\pm$ 1.4  & 7.1  \\ 
0534416-052357 & 17.8 $\pm$ 1.1  & 6.3  \\ 
0534458-054812 & 23.2 $\pm$ 1.3  & 6.7  \\ 
0534465-052325 & 20.5 $\pm$ 1.6  & 4.1  \\ 
0534467-052604 & 16.0 $\pm$ 0.8  & 7.0  \\ 
0534468-052129 & 19.4 $\pm$ 1.3  & 6.2  \\ 
0534478-053046 & 24.8 $\pm$ 0.5  & 17.6  \\ 
0534481-052238 & 14.5 $\pm$ 1.3  & 4.6  \\ 
0534482-053235 & 20.0 $\pm$ 0.7  & 8.3  \\ 
0534489-052816 & 16.3 $\pm$ 1.0  & 8.5  \\ 
0534507-052701 & 23.9 $\pm$ 0.6  & 16.0  \\ 
0534509-051756 & 15.5 $\pm$ 1.2  & 6.2  \\ 
0534514-051329 & 15.9 $\pm$ 1.6  & 7.2  \\ 
0534515-052513 & 24.1 $\pm$ 0.5  & 20.6  \\ 
0534517-053924 & 19.8 $\pm$ 0.7  & 13.5  \\ 
0534522-051203 & 29.8 $\pm$ 0.7  & 12.9  \\ 
0534526-052945 & 22.9 $\pm$ 1.0  & 12.4  \\ 
0534533-055405 & -24.9 $\pm$ 1.7  & 4.2  \\ 
0534541-052854 & 18.6 $\pm$ 1.1  & 6.4  \\ 
0534565-052751 & 24.4 $\pm$ 0.6  & 16.1  \\ 
0534568-051133 & 21.1 $\pm$ 0.2  & 46.6  \\ 
0534572-054202 & 25.0 $\pm$ 0.6  & 15.7  \\ 
0534577-052352 & 26.5 $\pm$ 0.3  & 36.2  \\ 
0534587-052117 & 19.2 $\pm$ 1.3  & 5.5  \\ 
0535007-053807 & -80.8 $\pm$ 1.4  & 4.2  \\ 
0535011-052406 & 25.8 $\pm$ 0.4  & 22.9  \\ 
0535021-052909 & 19.6 $\pm$ 0.6  & 16.0  \\ 
0535024-053309 & 25.6 $\pm$ 0.5  & 22.6  \\ 
0535031-050917 & 27.8 $\pm$ 1.9  & 4.8  \\ 
0535040-052637 & 23.5 $\pm$ 0.6  & 16.3  \\ 
0535040-054051 & 26.0 $\pm$ 0.5  & 16.8  \\ 
0535043-052313 & 36.4 $\pm$ 1.9  & 11.8  \\ 
0535045-052938 & 27.7 $\pm$ 0.3  & 32.2  \\ 
0535050-053643 & 20.0 $\pm$ 1.6  & 7.1  \\ 
0535056-045853 & 32.5 $\pm$ 0.4  & 22.4  \\ 
0535057-053355 & 20.4 $\pm$ 0.9  & 10.7  \\ 
0535064-052704 & 5.2 $\pm$ 1.5  & 4.0  \\ 
0535076-053658 & 17.1 $\pm$ 1.9  & 5.0  \\ 
0535088-053149 & 28.5 $\pm$ 0.9  & 9.7  \\ 
0535116-053101 & 13.1 $\pm$ 0.7  & 10.6  \\ 
0535119-054537 & 24.7 $\pm$ 0.4  & 27.7  \\ 
0535123-052347 & 27.0 $\pm$ 0.9  & 9.5  \\ 
0535128-051524 & 27.1 $\pm$ 0.6  & 16.4  \\ 
0535128-053907 & 25.5 $\pm$ 0.6  & 16.2  \\ 
0535163-053202 & 9.9 $\pm$ 0.9  & 8.1  \\ 
0535167-052403 & 2.0 $\pm$ 6.1  & 5.1  \\ 
0535174-053025 & 22.2 $\pm$ 0.5  & 18.6  \\ 
0535182-052846 & 25.1 $\pm$ 0.7  & 13.5  \\ 
0535188-051445 & 29.5 $\pm$ 0.8  & 12.7  \\ 
0535189-053736 & 29.1 $\pm$ 1.1  & 16.2  \\ 
0535198-053032 & 18.5 $\pm$ 1.2  & 5.0  \\ 
0535212-050916 & 30.4 $\pm$ 0.2  & 49.1  \\ 
0535218-050701 & 31.9 $\pm$ 0.5  & 19.5  \\ 
0535218-052353 & 22.8 $\pm$ 0.7  & 25.8  \\ 
0535226-051411 & 30.4 $\pm$ 1.3  & 8.8  \\ 
0535227-053136 & 21.2 $\pm$ 0.7  & 15.6  \\ 
0535242-052518 & 26.0 $\pm$ 1.3  & 7.9  \\ 
0535254-053403 & 19.6 $\pm$ 1.0  & 9.2  \\ 
0535256-053038 & 22.2 $\pm$ 1.1  & 6.0  \\ 
0535257-052935 & 12.5 $\pm$ 1.5  & 3.7  \\ 
0535263-052540 & 26.3 $\pm$ 1.3  & 22.5  \\ 
0535263-052743 & 19.8 $\pm$ 2.0  & 4.2  \\ 
0535280-051720 & 28.4 $\pm$ 1.5  & 5.5  \\ 
0535281-050049 & 53.2 $\pm$ 1.4  & 7.1  \\ 
0535291-052910 & 25.6 $\pm$ 0.5  & 21.3  \\ 
0535293-054538 & 25.7 $\pm$ 1.3  & 8.8  \\ 
0535298-051210 & 65.6 $\pm$ 5.6  & 3.9  \\ 
0535307-051807 & 26.9 $\pm$ 1.5  & 4.6  \\ 
0535321-051157 & 53.2 $\pm$ 3.3  & 4.5  \\ 
0535331-051410 & 30.9 $\pm$ 2.1  & 3.9  \\ 
0535333-053924 & 25.6 $\pm$ 0.8  & 12.5  \\ 
0535342-052718 & 26.9 $\pm$ 4.8  & 5.0  \\ 
0535346-053438 & 26.7 $\pm$ 0.6  & 15.7  \\ 
0535353-051111 & 25.0 $\pm$ 3.5  & 4.9  \\ 
0535355-051543 & 26.4 $\pm$ 0.5  & 21.3  \\ 
0535359-051225 & 39.0 $\pm$ 3.8  & 4.1  \\ 
0535359-053842 & 30.1 $\pm$ 1.3  & 9.0  \\ 
0535388-051242 & 30.2 $\pm$ 0.5  & 23.2  \\ 
0535426-052608 & 11.6 $\pm$ 1.7  & 4.1  \\ 
0535445-053633 & 19.1 $\pm$ 1.5  & 5.5  \\ 
0535448-052434 & 24.4 $\pm$ 1.1  & 9.8  \\ 
0535453-052810 & 25.6 $\pm$ 1.5  & 6.0  \\ 
0535462-051539 & 29.2 $\pm$ 2.2  & 3.8  \\ 
0535462-051808 & 26.4 $\pm$ 0.7  & 14.0  \\ 
0535505-055142 & 26.7 $\pm$ 0.3  & 27.3  \\ 
0535526-050505 & 29.4 $\pm$ 0.3  & 47.0  \\ 
0535530-055041 & 36.3 $\pm$ 0.8  & 9.7  \\ 
0535543-052644 & 27.3 $\pm$ 1.0  & 10.8  \\ 
0536038-053018 & 23.5 $\pm$ 1.2  & 6.2  \\ 
0536066-054154 & 28.3 $\pm$ 2.1  & 6.7  \\ 
0536114-053851 & 12.0 $\pm$ 2.4  & 5.2  \\ 
0536197-051438 & 30.6 $\pm$ 1.6  & 3.9  \\ 
0536213-052014 & 23.4 $\pm$ 0.6  & 16.5  \\ 
0536251-051913 & 19.6 $\pm$ 1.6  & 5.5  \\ 
0536255-051841 & 16.6 $\pm$ 1.4  & 5.6  \\ 
0536269-052505 & 21.3 $\pm$ 0.5  & 16.9  \\ 
0536275-053055 & 25.9 $\pm$ 0.6  & 16.3  \\ 
0536289-051443 & 27.5 $\pm$ 2.4  & 5.0  \\ 
0536321-051713 & 24.9 $\pm$ 1.3  & 7.1  \\ 
0536360-051135 & 21.2 $\pm$ 0.9  & 9.2  \\ 
0536482-052257 & 11.1 $\pm$ 1.0  & 8.4  \\ 

\enddata
\end{deluxetable}


==> tab7-full.tex <==
\begin{deluxetable}{lllll}
\rotate
\tablewidth{0pt}

\tabletypesize{\scriptsize}
\tablecaption{MIKE Field A Velocity Data}
\tablehead{
  \colhead{2massID} &  \colhead{RV A\_1} & \colhead{RV A\_2} & \colhead{R A\_1} &\colhead{R A\_2}  \\
    \colhead{}    &  \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & & \\

   }
\startdata
0534330-055747 & -2.4 $\pm$ 3.6  & 59.8 $\pm$ 1.9  & 4.6 & 9.4 \\ 
0534338-055638 & -7.4 $\pm$ 2.5  & -3.8 $\pm$ 1.4  & 6.9 & 13.6 \\ 
0534347-055308 & 0.0 $\pm$ 0.0  & 112.3 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0534351-055815 & 23.0 $\pm$ 2.6  & 25.1 $\pm$ 2.7  & 6.9 & 6.4 \\ 
0534377-060233 & 26.4 $\pm$ 1.5  & 24.1 $\pm$ 1.0  & 12.4 & 20.3 \\ 
0534389-055753 & 25.4 $\pm$ 1.5  & 23.2 $\pm$ 0.9  & 12.8 & 21.5 \\ 
0534392-055056 & 28.3 $\pm$ 3.0  & 29.4 $\pm$ 1.6  & 5.7 & 11.6 \\ 
0534401-060219 & 72.6 $\pm$ 4.1  & 0.0 $\pm$ 0.0  & 3.9 & 0.0 \\ 
0534411-055437 & 0.0 $\pm$ 0.0  & 22.1 $\pm$ 2.9  & 0.0 & 5.8 \\ 
0534420-055852 & 24.3 $\pm$ 2.6  & 22.7 $\pm$ 3.0  & 6.9 & 5.7 \\ 
0534435-055810 & 59.1 $\pm$ 1.4  & 57.1 $\pm$ 1.4  & 13.2 & 13.1 \\ 
0534444-055614 & 0.0 $\pm$ 0.0  & 48.5 $\pm$ 2.1  & 0.0 & 8.7 \\ 
0534456-055848 & 33.4 $\pm$ 3.5  & 33.1 $\pm$ 4.4  & 4.7 & 3.6 \\ 
0534461-060532 & 0.0 $\pm$ 0.0  & -8.4 $\pm$ 4.1  & 0.0 & 4.0 \\ 
0534469-055220 & 24.6 $\pm$ 3.4  & 27.4 $\pm$ 2.9  & 5.0 & 5.9 \\ 
0534469-060448 & 17.2 $\pm$ 3.4  & 38.3 $\pm$ 4.2  & 4.8 & 3.7 \\ 
0534475-055756 & -24.8 $\pm$ 2.2  & -27.6 $\pm$ 1.9  & 8.2 & 9.6 \\ 
0534483-055159 & 24.0 $\pm$ 2.6  & 22.8 $\pm$ 3.0  & 6.8 & 5.8 \\ 
0534487-060407 & 0.0 $\pm$ 0.0  & 20.9 $\pm$ 3.5  & 0.0 & 4.8 \\ 
0534492-060011 & 59.1 $\pm$ 2.3  & 78.2 $\pm$ 1.8  & 7.6 & 10.2 \\ 
0534500-055333 & 24.8 $\pm$ 1.6  & 32.4 $\pm$ 4.1  & 12.1 & 3.9 \\ 
0534515-060344 & 0.0 $\pm$ 0.0  & 28.8 $\pm$ 3.7  & 0.0 & 4.4 \\ 
0534520-060320 & 25.6 $\pm$ 2.5  & 24.9 $\pm$ 3.9  & 7.2 & 4.1 \\ 
0534528-060335 & 41.6 $\pm$ 1.9  & 38.1 $\pm$ 1.0  & 9.6 & 20.0 \\ 
0534531-054742 & 21.1 $\pm$ 2.8  & 28.7 $\pm$ 2.2  & 6.3 & 8.1 \\ 
0534533-055405 & 0.0 $\pm$ 0.0  & 181.2 $\pm$ 3.9  & 0.0 & 4.1 \\ 
0534533-055805 & 0.0 $\pm$ 0.0  & 26.1 $\pm$ 2.4  & 0.0 & 7.2 \\ 
0534536-055907 & 26.7 $\pm$ 1.1  & 0.0 $\pm$ 0.0  & 19.3 & 0.0 \\ 
0534542-060550 & 53.0 $\pm$ 1.5  & 45.4 $\pm$ 1.6  & 12.5 & 12.0 \\ 
0534543-055721 & 0.0 $\pm$ 0.0  & 168.8 $\pm$ 3.7  & 0.0 & 4.4 \\ 
0534543-060202 & 22.0 $\pm$ 2.8  & 20.3 $\pm$ 2.5  & 6.0 & 7.1 \\ 
0534549-054708 & 79.9 $\pm$ 1.5  & 79.9 $\pm$ 1.6  & 12.9 & 12.3 \\ 
0534556-055529 & 21.4 $\pm$ 2.1  & 21.6 $\pm$ 1.2  & 8.7 & 16.7 \\ 
0534556-060103 & 17.9 $\pm$ 2.2  & 12.4 $\pm$ 1.9  & 8.0 & 9.8 \\ 
0534560-054935 & 0.0 $\pm$ 0.0  & 24.8 $\pm$ 2.1  & 0.0 & 8.6 \\ 
0534565-055206 & 8.4 $\pm$ 2.2  & 7.7 $\pm$ 1.4  & 8.3 & 13.2 \\ 
0534571-060316 & 17.6 $\pm$ 1.3  & 14.8 $\pm$ 2.5  & 15.2 & 7.0 \\ 
0534575-055032 & 112.8 $\pm$ 3.5  & 115.6 $\pm$ 3.9  & 4.8 & 4.1 \\ 
0534576-054819 & 0.0 $\pm$ 0.0  & 49.2 $\pm$ 4.5  & 0.0 & 3.5 \\ 
0534579-054842 & 18.3 $\pm$ 2.8  & 0.0 $\pm$ 0.0  & 6.2 & 0.0 \\ 
0534579-055321 & 23.9 $\pm$ 2.9  & 27.0 $\pm$ 2.6  & 6.0 & 6.6 \\ 
0534582-054934 & 24.6 $\pm$ 2.5  & 24.5 $\pm$ 2.7  & 7.1 & 6.4 \\ 
0534583-055428 & 22.8 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 3.6 & 0.0 \\ 
0534585-060000 & 25.4 $\pm$ 1.0  & 25.4 $\pm$ 1.2  & 19.5 & 16.4 \\ 
0534588-054706 & 15.8 $\pm$ 3.3  & 22.1 $\pm$ 2.7  & 5.0 & 6.4 \\ 
0534593-060722 & 59.5 $\pm$ 3.5  & 58.1 $\pm$ 2.9  & 4.7 & 6.0 \\ 
0535001-060101 & 70.7 $\pm$ 0.8  & 74.4 $\pm$ 0.8  & 26.6 & 27.7 \\ 
0535005-054859 & 25.0 $\pm$ 3.9  & 21.5 $\pm$ 4.1  & 4.2 & 3.9 \\ 
0535005-060123 & 0.0 $\pm$ 0.0  & 25.0 $\pm$ 2.5  & 0.0 & 7.1 \\ 
0535013-055554 & 23.5 $\pm$ 3.7  & 27.8 $\pm$ 3.2  & 4.4 & 5.3 \\ 
0535013-060355 & 26.8 $\pm$ 3.2  & 27.4 $\pm$ 2.6  & 5.2 & 6.7 \\ 
0535014-060819 & 21.9 $\pm$ 3.3  & 27.2 $\pm$ 3.3  & 5.1 & 5.1 \\ 
0535016-055418 & 24.9 $\pm$ 2.2  & 28.6 $\pm$ 1.7  & 8.1 & 10.9 \\ 
0535018-054932 & 24.3 $\pm$ 2.2  & 28.1 $\pm$ 2.2  & 8.4 & 8.2 \\ 
0535021-054720 & 28.0 $\pm$ 3.1  & 24.1 $\pm$ 3.4  & 5.5 & 5.0 \\ 
0535028-055103 & 21.6 $\pm$ 2.8  & 23.5 $\pm$ 4.1  & 6.2 & 3.8 \\ 
0535029-060525 & 26.7 $\pm$ 2.8  & 28.7 $\pm$ 2.3  & 6.2 & 7.7 \\ 
0535035-055158 & 20.5 $\pm$ 4.3  & 56.0 $\pm$ 4.2  & 3.7 & 3.8 \\ 
0535039-055401 & 24.3 $\pm$ 2.3  & 23.6 $\pm$ 1.7  & 7.6 & 10.7 \\ 
0535040-054854 & 0.0 $\pm$ 0.0  & 29.6 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0535043-060053 & 21.8 $\pm$ 3.0  & 20.6 $\pm$ 1.7  & 5.7 & 10.6 \\ 
0535047-055346 & 29.0 $\pm$ 2.5  & 30.9 $\pm$ 3.4  & 7.3 & 4.9 \\ 
0535057-060007 & 27.2 $\pm$ 2.9  & 30.6 $\pm$ 3.1  & 5.9 & 5.4 \\ 
0535060-055239 & 12.9 $\pm$ 2.7  & 0.0 $\pm$ 0.0  & 6.3 & 0.0 \\ 
0535065-055951 & 36.1 $\pm$ 3.1  & 21.3 $\pm$ 3.8  & 5.5 & 4.3 \\ 
0535067-055101 & 23.9 $\pm$ 2.9  & 21.6 $\pm$ 2.0  & 5.9 & 9.2 \\ 
0535067-055811 & 0.0 $\pm$ 0.0  & 21.9 $\pm$ 1.3  & 0.0 & 15.0 \\ 
0535073-054801 & 26.2 $\pm$ 2.8  & 22.3 $\pm$ 1.5  & 6.3 & 12.8 \\ 
0535073-055606 & -10.2 $\pm$ 3.1  & -10.8 $\pm$ 1.4  & 5.5 & 13.6 \\ 
0535076-055208 & 25.1 $\pm$ 1.4  & 23.2 $\pm$ 1.2  & 13.5 & 15.6 \\ 
0535076-060654 & 21.9 $\pm$ 3.1  & 27.6 $\pm$ 2.7  & 5.5 & 6.5 \\ 
0535080-054853 & 26.4 $\pm$ 2.1  & 24.9 $\pm$ 1.2  & 8.6 & 16.2 \\ 
0535082-055000 & 25.5 $\pm$ 4.4  & 25.4 $\pm$ 2.5  & 3.5 & 7.0 \\ 
0535086-060502 & 0.0 $\pm$ 0.0  & -170.3 $\pm$ 3.7  & 0.0 & 4.4 \\ 
0535089-055817 & 25.5 $\pm$ 2.6  & 19.3 $\pm$ 3.0  & 6.6 & 5.6 \\ 
0535099-055711 & 21.5 $\pm$ 2.7  & 29.3 $\pm$ 1.8  & 6.3 & 10.2 \\ 
0535100-060536 & 24.0 $\pm$ 1.6  & 23.8 $\pm$ 1.5  & 11.9 & 12.9 \\ 
0535101-054834 & 46.7 $\pm$ 4.3  & 25.9 $\pm$ 2.2  & 3.6 & 8.1 \\ 
0535103-054633 & 23.1 $\pm$ 3.9  & 0.0 $\pm$ 0.0  & 4.2 & 0.0 \\ 
0535106-060144 & 26.7 $\pm$ 3.6  & 19.1 $\pm$ 2.4  & 4.5 & 7.4 \\ 
0535111-060021 & 27.7 $\pm$ 1.6  & 28.2 $\pm$ 1.4  & 11.7 & 13.8 \\ 
0535120-054729 & 26.1 $\pm$ 1.3  & 21.8 $\pm$ 1.1  & 15.6 & 18.5 \\ 
0535123-055607 & 24.1 $\pm$ 1.0  & 23.3 $\pm$ 1.1  & 19.7 & 18.2 \\ 
0535125-055128 & 23.9 $\pm$ 2.3  & 20.5 $\pm$ 2.0  & 7.8 & 8.9 \\ 
0535125-055708 & 23.8 $\pm$ 3.0  & 25.9 $\pm$ 4.1  & 5.7 & 3.9 \\ 
0535126-060110 & 23.8 $\pm$ 1.1  & 24.8 $\pm$ 1.0  & 17.8 & 19.7 \\ 
0535128-055526 & 34.1 $\pm$ 1.3  & 42.8 $\pm$ 1.2  & 15.5 & 16.9 \\ 
0535129-055938 & 27.8 $\pm$ 3.5  & 21.1 $\pm$ 4.0  & 4.7 & 4.1 \\ 
0535139-060008 & 0.0 $\pm$ 0.0  & 18.0 $\pm$ 2.2  & 0.0 & 8.1 \\ 
0535144-055426 & 31.2 $\pm$ 2.4  & 0.0 $\pm$ 0.0  & 7.4 & 0.0 \\ 
0535144-060512 & -142.5 $\pm$ 4.2  & 0.0 $\pm$ 0.0  & 3.7 & 0.0 \\ 
0535147-055104 & 25.4 $\pm$ 2.9  & 26.6 $\pm$ 2.3  & 6.0 & 7.9 \\ 
0535148-055142 & 25.2 $\pm$ 1.6  & 23.3 $\pm$ 1.5  & 11.8 & 12.9 \\ 
0535149-054934 & 23.9 $\pm$ 3.4  & 24.4 $\pm$ 2.1  & 4.9 & 8.7 \\ 
0535149-055636 & 25.5 $\pm$ 1.5  & 24.9 $\pm$ 1.4  & 12.9 & 14.1 \\ 
0535151-055305 & 25.2 $\pm$ 1.3  & 28.7 $\pm$ 1.6  & 15.1 & 11.6 \\ 
0535153-060137 & 24.3 $\pm$ 2.1  & 25.8 $\pm$ 1.4  & 8.7 & 13.4 \\ 
0535153-060630 & 21.9 $\pm$ 1.2  & 23.6 $\pm$ 1.0  & 15.9 & 20.5 \\ 
0535157-060939 & 12.0 $\pm$ 0.8  & 11.2 $\pm$ 0.8  & 28.8 & 27.1 \\ 
0535160-055044 & 26.0 $\pm$ 2.3  & 28.5 $\pm$ 1.6  & 7.7 & 11.5 \\ 
0535160-060438 & 24.6 $\pm$ 2.3  & 25.5 $\pm$ 1.8  & 7.8 & 10.5 \\ 
0535169-054555 & 23.4 $\pm$ 1.4  & 23.4 $\pm$ 1.3  & 13.5 & 14.1 \\ 
0535170-055830 & 24.0 $\pm$ 1.9  & 22.8 $\pm$ 2.1  & 9.8 & 8.5 \\ 
0535170-055931 & 14.2 $\pm$ 0.9  & 16.3 $\pm$ 0.8  & 25.6 & 27.3 \\ 
0535173-060515 & 23.6 $\pm$ 2.2  & 21.9 $\pm$ 2.8  & 8.0 & 6.1 \\ 
0535176-055213 & 23.7 $\pm$ 2.6  & 27.7 $\pm$ 2.0  & 6.8 & 9.1 \\ 
0535177-055645 & 22.2 $\pm$ 2.4  & 21.8 $\pm$ 2.4  & 7.4 & 7.5 \\ 
0535179-054937 & 24.8 $\pm$ 1.5  & 24.1 $\pm$ 1.4  & 12.4 & 13.0 \\ 
0535189-055615 & 20.2 $\pm$ 1.3  & 21.6 $\pm$ 1.4  & 14.9 & 13.4 \\ 
0535190-054616 & 25.8 $\pm$ 1.3  & 24.7 $\pm$ 1.6  & 15.2 & 11.9 \\ 
0535191-060437 & 26.1 $\pm$ 2.5  & 24.1 $\pm$ 2.9  & 7.1 & 6.0 \\ 
0535192-054701 & 25.1 $\pm$ 2.8  & 30.8 $\pm$ 1.8  & 6.3 & 10.2 \\ 
0535193-054802 & 0.0 $\pm$ 0.0  & 77.5 $\pm$ 1.6  & 0.0 & 12.0 \\ 
0535200-054552 & 24.4 $\pm$ 2.2  & 27.0 $\pm$ 2.2  & 8.2 & 8.3 \\ 
0535208-060717 & 24.6 $\pm$ 1.9  & 26.8 $\pm$ 1.9  & 9.9 & 9.8 \\ 
0535209-060400 & 0.0 $\pm$ 0.0  & -104.5 $\pm$ 4.2  & 0.0 & 3.8 \\ 
0535210-055534 & 28.8 $\pm$ 4.1  & 0.0 $\pm$ 0.0  & 4.0 & 0.0 \\ 
0535213-055635 & 25.5 $\pm$ 1.5  & 24.3 $\pm$ 1.3  & 12.6 & 14.6 \\ 
0535218-054608 & 0.0 $\pm$ 0.0  & 27.0 $\pm$ 4.0  & 0.0 & 4.0 \\ 
0535219-055405 & 23.6 $\pm$ 1.2  & 24.9 $\pm$ 1.2  & 15.5 & 16.7 \\ 
0535220-055236 & 22.3 $\pm$ 2.0  & 28.0 $\pm$ 1.7  & 9.2 & 11.0 \\ 
0535231-055543 & 26.7 $\pm$ 1.2  & 24.6 $\pm$ 1.0  & 16.3 & 20.5 \\ 
0535232-060158 & 0.0 $\pm$ 0.0  & 25.2 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0535232-060301 & 25.8 $\pm$ 1.3  & 25.1 $\pm$ 1.4  & 15.2 & 13.8 \\ 
0535232-060452 & 25.3 $\pm$ 2.5  & 27.2 $\pm$ 2.0  & 7.2 & 9.2 \\ 
0535238-055127 & -24.2 $\pm$ 2.2  & -24.0 $\pm$ 2.0  & 8.2 & 9.2 \\ 
0535239-055941 & 29.9 $\pm$ 4.5  & 22.7 $\pm$ 3.7  & 3.5 & 4.3 \\ 
0535244-060146 & 25.0 $\pm$ 4.3  & 20.9 $\pm$ 3.6  & 3.7 & 4.5 \\ 
0535247-060459 & 22.7 $\pm$ 1.6  & 18.7 $\pm$ 1.7  & 11.5 & 10.7 \\ 
0535251-055739 & 25.2 $\pm$ 1.7  & 26.0 $\pm$ 1.8  & 10.7 & 10.3 \\ 
0535254-055108 & 27.6 $\pm$ 2.7  & 26.4 $\pm$ 2.2  & 6.3 & 8.1 \\ 
0535264-055526 & 22.3 $\pm$ 2.3  & 20.2 $\pm$ 2.0  & 7.9 & 9.2 \\ 
0535265-054849 & 28.9 $\pm$ 1.3  & 28.9 $\pm$ 1.6  & 14.2 & 11.5 \\ 
0535278-055634 & 24.4 $\pm$ 1.2  & 23.2 $\pm$ 1.3  & 16.2 & 15.1 \\ 
0535279-060939 & 24.6 $\pm$ 2.9  & 27.1 $\pm$ 1.5  & 5.9 & 12.9 \\ 
0535283-055913 & 19.2 $\pm$ 1.9  & 17.6 $\pm$ 2.2  & 9.4 & 8.0 \\ 
0535290-054948 & 24.9 $\pm$ 1.5  & 22.4 $\pm$ 1.3  & 13.0 & 14.1 \\ 
0535291-055502 & 29.3 $\pm$ 3.4  & 29.3 $\pm$ 3.3  & 5.0 & 5.2 \\ 
0535293-054538 & 10.1 $\pm$ 3.4  & 7.0 $\pm$ 4.1  & 4.9 & 3.9 \\ 
0535298-060739 & -31.7 $\pm$ 2.2  & -34.2 $\pm$ 1.8  & 8.2 & 10.3 \\ 
0535301-055426 & 24.0 $\pm$ 0.9  & 21.9 $\pm$ 0.9  & 22.3 & 22.3 \\ 
0535301-060302 & 12.5 $\pm$ 4.4  & -101.4 $\pm$ 4.4  & 3.6 & 3.5 \\ 
0535302-055116 & 26.4 $\pm$ 1.0  & 24.7 $\pm$ 1.3  & 18.7 & 14.2 \\ 
0535304-054903 & -100.1 $\pm$ 4.2  & 17.1 $\pm$ 3.9  & 3.8 & 4.2 \\ 
0535304-060500 & 5.5 $\pm$ 2.9  & 24.9 $\pm$ 1.0  & 5.9 & 19.6 \\ 
0535305-055155 & 23.2 $\pm$ 4.2  & 26.0 $\pm$ 4.0  & 3.7 & 4.0 \\ 
0535309-055542 & 17.4 $\pm$ 1.5  & 16.3 $\pm$ 1.3  & 12.6 & 15.0 \\ 
0535313-055840 & 27.5 $\pm$ 1.7  & 29.9 $\pm$ 1.6  & 11.2 & 11.9 \\ 
0535325-060122 & 24.7 $\pm$ 3.0  & 22.6 $\pm$ 2.4  & 5.7 & 7.2 \\ 
0535326-054528 & 26.5 $\pm$ 1.2  & 23.4 $\pm$ 1.7  & 16.0 & 10.7 \\ 
0535329-054932 & 23.2 $\pm$ 3.4  & 26.0 $\pm$ 3.2  & 5.0 & 5.4 \\ 
0535329-055802 & 24.5 $\pm$ 1.6  & 27.2 $\pm$ 1.1  & 11.8 & 16.9 \\ 
0535331-054707 & 0.0 $\pm$ 0.0  & 26.9 $\pm$ 3.6  & 0.0 & 4.6 \\ 
0535332-055856 & 21.8 $\pm$ 1.1  & 30.4 $\pm$ 1.2  & 19.4 & 16.5 \\ 
0535335-060220 & 29.8 $\pm$ 4.1  & 27.1 $\pm$ 3.0  & 3.9 & 5.7 \\ 
0535338-054821 & 23.3 $\pm$ 3.4  & 28.6 $\pm$ 3.3  & 5.0 & 5.2 \\ 
0535340-055505 & 0.0 $\pm$ 0.0  & 122.3 $\pm$ 4.0  & 0.0 & 4.1 \\ 
0535346-060247 & 27.0 $\pm$ 1.8  & 24.7 $\pm$ 1.4  & 10.0 & 13.9 \\ 
0535355-055819 & 56.3 $\pm$ 3.8  & 21.3 $\pm$ 2.0  & 4.3 & 9.1 \\ 
0535361-055513 & 37.2 $\pm$ 3.5  & 30.6 $\pm$ 3.9  & 4.8 & 4.2 \\ 
0535361-055653 & 23.4 $\pm$ 1.6  & 26.6 $\pm$ 2.0  & 12.1 & 9.0 \\ 
0535367-055856 & 26.9 $\pm$ 1.7  & 26.1 $\pm$ 1.2  & 10.6 & 15.4 \\ 
0535373-060000 & 5.3 $\pm$ 3.8  & 34.2 $\pm$ 3.8  & 4.3 & 4.3 \\ 
0535374-055128 & 22.3 $\pm$ 1.6  & 23.5 $\pm$ 2.1  & 11.9 & 8.6 \\ 
0535384-055245 & 0.0 $\pm$ 0.0  & 39.6 $\pm$ 4.2  & 0.0 & 3.8 \\ 
0535391-055806 & 67.9 $\pm$ 1.9  & 67.0 $\pm$ 1.1  & 9.9 & 18.9 \\ 
0535397-055655 & 28.3 $\pm$ 1.8  & 24.9 $\pm$ 2.6  & 10.2 & 6.8 \\ 
0535405-055803 & 25.1 $\pm$ 3.0  & 25.9 $\pm$ 2.9  & 5.7 & 5.8 \\ 
0535405-055826 & 27.8 $\pm$ 2.3  & 25.4 $\pm$ 2.3  & 7.8 & 7.8 \\ 
0535418-055229 & -0.5 $\pm$ 4.2  & 0.0 $\pm$ 0.0  & 3.8 & 0.0 \\ 
0535428-055136 & 22.8 $\pm$ 2.5  & 26.0 $\pm$ 1.9  & 6.9 & 9.4 \\ 
0535430-055945 & -21.6 $\pm$ 1.6  & -25.4 $\pm$ 2.9  & 11.8 & 6.0 \\ 
0535440-055653 & 27.7 $\pm$ 3.8  & 22.9 $\pm$ 2.9  & 4.3 & 5.8 \\ 
0535441-055004 & 23.2 $\pm$ 2.1  & 23.0 $\pm$ 3.5  & 8.6 & 4.7 \\ 
0535447-055102 & 25.4 $\pm$ 1.4  & 25.4 $\pm$ 1.5  & 14.0 & 12.5 \\ 
0535451-060107 & 188.3 $\pm$ 3.3  & 0.0 $\pm$ 0.0  & 5.0 & 0.0 \\ 
0535454-055600 & 0.0 $\pm$ 0.0  & -80.8 $\pm$ 3.9  & 0.0 & 4.2 \\ 
0535455-055730 & 29.4 $\pm$ 2.3  & 24.0 $\pm$ 2.3  & 8.0 & 7.8 \\ 
0535458-060538 & -14.6 $\pm$ 4.4  & 24.1 $\pm$ 2.7  & 3.6 & 6.5 \\ 
0535466-054926 & 24.7 $\pm$ 1.5  & 24.1 $\pm$ 1.4  & 12.6 & 13.9 \\ 
0535468-060507 & 0.0 $\pm$ 0.0  & -17.8 $\pm$ 4.3  & 0.0 & 3.7 \\ 
0535473-055511 & 26.1 $\pm$ 2.2  & 21.0 $\pm$ 3.5  & 8.1 & 4.7 \\ 
0535474-060027 & 26.2 $\pm$ 1.6  & 24.1 $\pm$ 1.4  & 12.1 & 13.8 \\ 
0535476-055806 & 26.4 $\pm$ 3.0  & 27.3 $\pm$ 3.1  & 5.8 & 5.5 \\ 
0535479-060134 & 0.0 $\pm$ 0.0  & 25.3 $\pm$ 3.4  & 0.0 & 5.0 \\ 
0535481-055357 & 24.0 $\pm$ 2.9  & 20.5 $\pm$ 2.5  & 5.9 & 7.0 \\ 
0535483-055011 & 35.7 $\pm$ 1.0  & 32.5 $\pm$ 1.1  & 20.5 & 19.2 \\ 
0535485-055623 & 27.1 $\pm$ 3.7  & 28.3 $\pm$ 2.8  & 4.5 & 6.1 \\ 
0535485-060525 & 22.8 $\pm$ 3.1  & 17.5 $\pm$ 3.2  & 5.6 & 5.3 \\ 
0535530-055041 & 26.7 $\pm$ 2.0  & 26.2 $\pm$ 3.6  & 9.3 & 4.6 \\ 
0535546-055436 & 27.3 $\pm$ 2.9  & 24.3 $\pm$ 2.6  & 5.9 & 6.8 \\ 
0535550-055420 & 25.7 $\pm$ 1.2  & 22.8 $\pm$ 1.2  & 16.3 & 16.6 \\ 
0535561-055228 & 26.8 $\pm$ 1.9  & 23.2 $\pm$ 1.9  & 9.9 & 9.8 \\ 
0535573-060224 & 29.7 $\pm$ 1.4  & 28.9 $\pm$ 1.6  & 14.0 & 12.2 \\ 
0535576-055718 & 0.0 $\pm$ 0.0  & 33.5 $\pm$ 4.2  & 0.0 & 3.8 \\ 
0535589-055908 & 23.1 $\pm$ 1.3  & 20.8 $\pm$ 1.4  & 14.3 & 13.6 \\ 
0535589-060239 & 26.6 $\pm$ 1.8  & 25.4 $\pm$ 1.7  & 10.6 & 10.8 \\ 
0536002-060329 & 13.9 $\pm$ 1.0  & 14.4 $\pm$ 0.9  & 20.4 & 22.3 \\ 
0536056-055213 & 19.9 $\pm$ 2.4  & 27.6 $\pm$ 2.9  & 7.3 & 6.0 \\ 
0536059-055254 & 31.8 $\pm$ 1.8  & 29.7 $\pm$ 3.0  & 10.7 & 5.8 \\ 
0536062-060315 & 24.4 $\pm$ 2.2  & 20.4 $\pm$ 2.8  & 8.1 & 6.2 \\ 
0536068-055914 & 32.1 $\pm$ 3.2  & 32.5 $\pm$ 3.2  & 5.2 & 5.3 \\ 
0536099-055720 & 94.3 $\pm$ 2.5  & 95.1 $\pm$ 2.3  & 7.1 & 7.8 \\ 
0536108-055649 & 25.5 $\pm$ 1.3  & 26.9 $\pm$ 1.2  & 14.8 & 16.0 \\ 
0536110-055726 & 27.3 $\pm$ 2.3  & 35.3 $\pm$ 3.2  & 7.7 & 5.3 \\ 
\enddata
\end{deluxetable}


==> tab8-full.tex <==
\begin{deluxetable}{lllll}
\rotate
\tablewidth{0pt}

\tabletypesize{\scriptsize}
\tablecaption{MIKE Field B Velocity Data}
\tablehead{
  \colhead{2massID} &  \colhead{RV B\_1} & \colhead{RV B\_2} & \colhead{R B\_1} &\colhead{R B\_2}  \\
    \colhead{}    &  \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & & \\

   }
\startdata
0534174-053158 & 0.0 $\pm$ 0.0  & 26.2 $\pm$ 4.3  & 0.0 & 3.7 \\ 
0534181-052833 & 6.3 $\pm$ 4.5  & 0.0 $\pm$ 0.0  & 3.5 & 0.0 \\ 
0534195-053019 & 5.1 $\pm$ 4.4  & 14.0 $\pm$ 3.2  & 3.5 & 5.5 \\ 
0534207-053235 & 29.1 $\pm$ 3.9  & 0.0 $\pm$ 0.0  & 4.2 & 0.0 \\ 
0534209-052448 & 0.0 $\pm$ 0.0  & 33.8 $\pm$ 3.4  & 0.0 & 5.0 \\ 
0534224-052226 & 0.0 $\pm$ 0.0  & -27.0 $\pm$ 4.0  & 0.0 & 4.1 \\ 
0534265-052323 & 29.6 $\pm$ 3.3  & 26.7 $\pm$ 3.2  & 5.2 & 5.5 \\ 
0534279-052634 & 35.1 $\pm$ 3.4  & 0.0 $\pm$ 0.0  & 5.0 & 0.0 \\ 
0534285-052457 & 24.7 $\pm$ 2.7  & 23.5 $\pm$ 1.2  & 6.5 & 19.2 \\ 
0534311-052155 & 0.0 $\pm$ 0.0  & 169.0 $\pm$ 3.7  & 0.0 & 4.4 \\ 
0534316-052826 & 26.5 $\pm$ 2.1  & 27.7 $\pm$ 3.7  & 8.6 & 4.5 \\ 
0534318-053519 & 24.5 $\pm$ 1.4  & 0.0 $\pm$ 0.0  & 13.7 & 0.0 \\ 
0534327-052107 & 0.0 $\pm$ 0.0  & 33.6 $\pm$ 4.0  & 0.0 & 4.0 \\ 
0534352-053432 & 0.0 $\pm$ 0.0  & -28.7 $\pm$ 3.1  & 0.0 & 5.6 \\ 
0534356-053552 & 26.7 $\pm$ 3.5  & 26.3 $\pm$ 2.3  & 4.7 & 8.0 \\ 
0534358-053645 & 0.0 $\pm$ 0.0  & -31.1 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0534359-051524 & 25.9 $\pm$ 2.9  & 21.7 $\pm$ 2.0  & 6.0 & 9.7 \\ 
0534374-053451 & 0.0 $\pm$ 0.0  & 28.0 $\pm$ 2.7  & 0.0 & 6.6 \\ 
0534381-052740 & 21.1 $\pm$ 1.7  & 21.4 $\pm$ 1.8  & 11.3 & 10.8 \\ 
0534382-052423 & 29.2 $\pm$ 3.5  & 27.8 $\pm$ 3.1  & 4.8 & 5.6 \\ 
0534400-052604 & 0.0 $\pm$ 0.0  & 197.7 $\pm$ 3.9  & 0.0 & 4.2 \\ 
0534408-052242 & -117.2 $\pm$ 4.0  & 0.0 $\pm$ 0.0  & 4.0 & 0.0 \\ 
0534408-052809 & 0.0 $\pm$ 0.0  & -26.7 $\pm$ 3.7  & 0.0 & 4.5 \\ 
0534416-052357 & 0.0 $\pm$ 0.0  & -27.2 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0534427-052837 & 0.0 $\pm$ 0.0  & 175.3 $\pm$ 4.3  & 0.0 & 3.7 \\ 
0534444-052606 & 0.0 $\pm$ 0.0  & -23.5 $\pm$ 4.4  & 0.0 & 3.5 \\ 
0534463-052431 & 0.0 $\pm$ 0.0  & 26.1 $\pm$ 2.1  & 0.0 & 9.0 \\ 
0534465-052325 & 0.0 $\pm$ 0.0  & -184.7 $\pm$ 4.1  & 0.0 & 4.0 \\ 
0534468-052129 & 28.4 $\pm$ 3.0  & 0.0 $\pm$ 0.0  & 5.7 & 0.0 \\ 
0534482-053235 & 0.0 $\pm$ 0.0  & -28.8 $\pm$ 4.5  & 0.0 & 3.5 \\ 
0534487-051907 & 0.0 $\pm$ 0.0  & 20.8 $\pm$ 4.3  & 0.0 & 3.7 \\ 
0534489-052816 & 34.6 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 3.6 & 0.0 \\ 
0534490-052626 & 0.0 $\pm$ 0.0  & -30.9 $\pm$ 3.8  & 0.0 & 4.3 \\ 
0534504-052020 & 0.0 $\pm$ 0.0  & 21.7 $\pm$ 3.8  & 0.0 & 4.3 \\ 
0534507-052701 & 78.9 $\pm$ 4.0  & 21.5 $\pm$ 4.4  & 4.0 & 3.6 \\ 
0534518-052138 & 0.0 $\pm$ 0.0  & 19.9 $\pm$ 3.1  & 0.0 & 5.6 \\ 
0534520-052418 & 24.4 $\pm$ 3.6  & 25.0 $\pm$ 4.5  & 4.6 & 3.5 \\ 
0534520-052442 & -187.7 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 3.7 & 0.0 \\ 
0534523-053008 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 4.2  & 0.0 & 3.8 \\ 
0534526-052945 & 0.0 $\pm$ 0.0  & 11.0 $\pm$ 4.4  & 0.0 & 3.5 \\ 
0534528-053348 & 0.0 $\pm$ 0.0  & -31.7 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0534529-052859 & 195.6 $\pm$ 4.0  & 0.0 $\pm$ 0.0  & 4.0 & 0.0 \\ 
0534548-052512 & 0.0 $\pm$ 0.0  & -30.1 $\pm$ 3.5  & 0.0 & 4.8 \\ 
0534556-052937 & 0.0 $\pm$ 0.0  & -35.0 $\pm$ 3.4  & 0.0 & 4.9 \\ 
0534567-052637 & 0.0 $\pm$ 0.0  & -26.0 $\pm$ 2.8  & 0.0 & 6.2 \\ 
0534574-053042 & 23.6 $\pm$ 3.0  & 0.0 $\pm$ 0.0  & 5.8 & 0.0 \\ 
0534577-052352 & 25.4 $\pm$ 3.3  & 27.6 $\pm$ 1.4  & 5.2 & 14.8 \\ 
0534585-053249 & 40.2 $\pm$ 4.5  & 0.0 $\pm$ 0.0  & 3.5 & 0.0 \\ 
0535001-052301 & 0.0 $\pm$ 0.0  & 27.4 $\pm$ 1.6  & 0.0 & 12.6 \\ 
0535002-051850 & -131.8 $\pm$ 4.4  & 0.0 $\pm$ 0.0  & 3.5 & 0.0 \\ 
0535011-052406 & 0.0 $\pm$ 0.0  & 28.2 $\pm$ 2.3  & 0.0 & 8.1 \\ 
0535012-052016 & 183.0 $\pm$ 4.4  & 28.8 $\pm$ 3.2  & 3.6 & 5.3 \\ 
0535020-051537 & 0.0 $\pm$ 0.0  & 30.0 $\pm$ 2.4  & 0.0 & 7.6 \\ 
0535020-051834 & 6.1 $\pm$ 4.5  & 0.0 $\pm$ 0.0  & 3.5 & 0.0 \\ 
0535021-052909 & 0.0 $\pm$ 0.0  & -178.4 $\pm$ 4.2  & 0.0 & 3.8 \\ 
0535024-052046 & 0.0 $\pm$ 0.0  & 23.8 $\pm$ 3.5  & 0.0 & 4.8 \\ 
0535030-052237 & 97.9 $\pm$ 3.9  & 0.0 $\pm$ 0.0  & 4.2 & 0.0 \\ 
0535032-051753 & 0.0 $\pm$ 0.0  & 58.3 $\pm$ 4.2  & 0.0 & 3.9 \\ 
0535035-052926 & 0.0 $\pm$ 0.0  & 27.6 $\pm$ 3.9  & 0.0 & 4.2 \\ 
0535039-051859 & -140.2 $\pm$ 4.4  & 0.0 $\pm$ 0.0  & 3.5 & 0.0 \\ 
0535039-052903 & 0.0 $\pm$ 0.0  & 42.6 $\pm$ 4.4  & 0.0 & 3.6 \\ 
0535043-052313 & -115.4 $\pm$ 4.2  & 29.1 $\pm$ 3.5  & 3.8 & 4.7 \\ 
0535045-052938 & 24.6 $\pm$ 3.8  & 25.0 $\pm$ 1.5  & 4.2 & 13.6 \\ 
0535053-052410 & 0.0 $\pm$ 0.0  & 33.2 $\pm$ 4.4  & 0.0 & 3.6 \\ 
0535053-053428 & 83.0 $\pm$ 3.9  & 0.0 $\pm$ 0.0  & 4.1 & 0.0 \\ 
0535056-051824 & 0.0 $\pm$ 0.0  & 29.7 $\pm$ 4.4  & 0.0 & 3.5 \\ 
0535056-052519 & 25.3 $\pm$ 1.7  & 18.5 $\pm$ 1.6  & 11.0 & 12.3 \\ 
0535064-052704 & 0.0 $\pm$ 0.0  & 168.2 $\pm$ 4.3  & 0.0 & 3.8 \\ 
0535080-053244 & 0.0 $\pm$ 0.0  & 34.3 $\pm$ 3.2  & 0.0 & 5.4 \\ 
0535088-053149 & 0.0 $\pm$ 0.0  & 25.7 $\pm$ 2.4  & 0.0 & 7.4 \\ 
0535101-052232 & 0.0 $\pm$ 0.0  & -113.4 $\pm$ 3.8  & 0.0 & 4.3 \\ 
0535105-052156 & 0.0 $\pm$ 0.0  & 24.7 $\pm$ 2.1  & 0.0 & 9.1 \\ 
0535105-053313 & 22.5 $\pm$ 4.4  & -27.6 $\pm$ 3.5  & 3.6 & 4.9 \\ 
0535125-052344 & 0.0 $\pm$ 0.0  & 24.1 $\pm$ 2.3  & 0.0 & 8.1 \\ 
0535128-051524 & 0.0 $\pm$ 0.0  & 26.9 $\pm$ 4.2  & 0.0 & 3.8 \\ 
0535130-053403 & -11.6 $\pm$ 4.4  & 0.0 $\pm$ 0.0  & 3.6 & 0.0 \\ 
0535135-051731 & 0.0 $\pm$ 0.0  & -24.1 $\pm$ 4.4  & 0.0 & 3.5 \\ 
0535140-051952 & 0.0 $\pm$ 0.0  & 24.0 $\pm$ 2.1  & 0.0 & 8.8 \\ 
0535142-052424 & 0.0 $\pm$ 0.0  & 23.7 $\pm$ 2.4  & 0.0 & 7.6 \\ 
0535144-052502 & 0.0 $\pm$ 0.0  & 66.3 $\pm$ 4.4  & 0.0 & 3.6 \\ 
0535149-053639 & 0.0 $\pm$ 0.0  & -30.7 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0535153-051902 & 0.0 $\pm$ 0.0  & -26.8 $\pm$ 3.5  & 0.0 & 4.9 \\ 
0535154-051738 & 0.0 $\pm$ 0.0  & -35.1 $\pm$ 3.8  & 0.0 & 4.3 \\ 
0535154-053511 & 33.5 $\pm$ 4.3  & -26.0 $\pm$ 4.4  & 3.7 & 3.6 \\ 
0535156-052403 & 0.0 $\pm$ 0.0  & 47.7 $\pm$ 3.4  & 0.0 & 4.9 \\ 
0535158-052040 & 163.8 $\pm$ 4.2  & 0.0 $\pm$ 0.0  & 3.8 & 0.0 \\ 
0535159-051459 & 0.0 $\pm$ 0.0  & 25.8 $\pm$ 2.6  & 0.0 & 7.0 \\ 
0535163-053202 & 0.0 $\pm$ 0.0  & -29.3 $\pm$ 3.0  & 0.0 & 5.7 \\ 
0535174-053025 & 0.0 $\pm$ 0.0  & 23.7 $\pm$ 2.7  & 0.0 & 6.5 \\ 
0535182-052846 & -109.7 $\pm$ 3.9  & 26.3 $\pm$ 3.5  & 4.2 & 4.8 \\ 
0535185-051820 & 0.0 $\pm$ 0.0  & 31.9 $\pm$ 3.4  & 0.0 & 4.9 \\ 
0535188-051445 & 0.0 $\pm$ 0.0  & 33.2 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0535192-051644 & 0.0 $\pm$ 0.0  & -119.4 $\pm$ 4.4  & 0.0 & 3.6 \\ 
0535195-052104 & 0.0 $\pm$ 0.0  & -25.5 $\pm$ 3.4  & 0.0 & 4.9 \\ 
0535202-053039 & 0.0 $\pm$ 0.0  & 26.4 $\pm$ 2.7  & 0.0 & 6.5 \\ 
0535208-052130 & 0.0 $\pm$ 0.0  & -181.4 $\pm$ 4.4  & 0.0 & 3.6 \\ 
0535209-051637 & 0.0 $\pm$ 0.0  & 23.0 $\pm$ 2.3  & 0.0 & 8.2 \\ 
0535210-052809 & 0.0 $\pm$ 0.0  & 28.5 $\pm$ 3.1  & 0.0 & 5.5 \\ 
0535211-051821 & 0.0 $\pm$ 0.0  & 25.4 $\pm$ 4.3  & 0.0 & 3.7 \\ 
0535213-052345 & 93.4 $\pm$ 4.2  & 0.0 $\pm$ 0.0  & 3.8 & 0.0 \\ 
0535216-052526 & 0.0 $\pm$ 0.0  & 22.3 $\pm$ 3.6  & 0.0 & 4.6 \\ 
0535218-052208 & 0.0 $\pm$ 0.0  & 93.2 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0535219-051704 & 30.0 $\pm$ 3.7  & 29.8 $\pm$ 2.8  & 4.4 & 6.2 \\ 
0535219-052827 & 0.0 $\pm$ 0.0  & 43.6 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0535222-051808 & 0.0 $\pm$ 0.0  & -29.6 $\pm$ 3.8  & 0.0 & 4.4 \\ 
0535222-053116 & 0.0 $\pm$ 0.0  & -26.0 $\pm$ 3.9  & 0.0 & 4.2 \\ 
0535224-052545 & 0.0 $\pm$ 0.0  & 184.1 $\pm$ 3.6  & 0.0 & 4.6 \\ 
0535227-053137 & 2.1 $\pm$ 3.9  & 20.4 $\pm$ 4.0  & 4.2 & 4.0 \\ 
0535237-051839 & -79.7 $\pm$ 3.8  & 0.0 $\pm$ 0.0  & 4.3 & 0.0 \\ 
0535249-052510 & 0.0 $\pm$ 0.0  & 193.9 $\pm$ 4.4  & 0.0 & 3.5 \\ 
0535250-052346 & 0.0 $\pm$ 0.0  & 79.2 $\pm$ 4.3  & 0.0 & 3.7 \\ 
0535254-053402 & 191.3 $\pm$ 4.2  & 0.0 $\pm$ 0.0  & 3.8 & 0.0 \\ 
0535256-053020 & 0.0 $\pm$ 0.0  & 24.1 $\pm$ 3.5  & 0.0 & 4.8 \\ 
0535267-051645 & 0.0 $\pm$ 0.0  & 135.8 $\pm$ 4.5  & 0.0 & 3.5 \\ 
0535270-051544 & 0.0 $\pm$ 0.0  & 26.1 $\pm$ 4.1  & 0.0 & 3.9 \\ 
0535279-051657 & 0.0 $\pm$ 0.0  & 31.4 $\pm$ 4.5  & 0.0 & 3.5 \\ 
0535284-051902 & 0.0 $\pm$ 0.0  & -28.4 $\pm$ 4.4  & 0.0 & 3.6 \\ 
0535289-051618 & 0.0 $\pm$ 0.0  & 36.3 $\pm$ 4.0  & 0.0 & 4.0 \\ 
0535291-052910 & 0.0 $\pm$ 0.0  & 20.8 $\pm$ 4.5  & 0.0 & 3.5 \\ 
0535294-051633 & 0.0 $\pm$ 0.0  & 27.7 $\pm$ 3.2  & 0.0 & 5.4 \\ 
0535307-053036 & 0.0 $\pm$ 0.0  & 30.7 $\pm$ 3.9  & 0.0 & 4.2 \\ 
0535312-051855 & 0.0 $\pm$ 0.0  & 26.1 $\pm$ 3.4  & 0.0 & 5.0 \\ 
0535338-053225 & 0.0 $\pm$ 0.0  & -17.3 $\pm$ 2.6  & 0.0 & 6.8 \\ 
0535346-053438 & 0.0 $\pm$ 0.0  & 21.7 $\pm$ 3.8  & 0.0 & 4.4 \\ 
0535351-052123 & 0.0 $\pm$ 0.0  & -22.0 $\pm$ 3.3  & 0.0 & 5.2 \\ 
0535363-053137 & 10.9 $\pm$ 4.1  & -3.1 $\pm$ 4.5  & 4.0 & 3.5 \\ 
0535424-052733 & 0.0 $\pm$ 0.0  & 20.7 $\pm$ 4.0  & 0.0 & 4.1 \\ 
0535430-052302 & 191.7 $\pm$ 3.6  & -25.5 $\pm$ 3.6  & 4.6 & 4.7 \\ 
0535448-052434 & -96.7 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 3.7 & 0.0 \\ 
0535474-052249 & 89.9 $\pm$ 4.2  & 0.0 $\pm$ 0.0  & 3.8 & 0.0 \\ 
\enddata
\end{deluxetable}


==> tab9-full.tex <==
\begin{deluxetable}{lllllll}
\rotate
\tablewidth{0pt}

\tabletypesize{\scriptsize}
\tablecaption{MIKE Field C Velocity Data}
\tablehead{
  \colhead{2massID} &  \colhead{RV C\_1} & \colhead{RV C\_2} & \colhead{RV C\_3} & \colhead{R C\_1} & \colhead{R C\_2} & \colhead{R C\_3} \\
    \colhead{}    &  \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)} & \colhead{(km s$^{-1}$)}& & & \\

   }
\startdata
0534269-051803 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & -24.5 $\pm$ 4.4  & 0.0 & 0.0 & 3.6\\ 
0534290-051414 & 25.7 $\pm$ 1.9  & 20.3 $\pm$ 2.0  & 21.4 $\pm$ 2.1  & 9.9 & 9.1 & 8.7\\ 
0534292-051439 & 28.2 $\pm$ 1.3  & 25.3 $\pm$ 1.3  & 26.3 $\pm$ 1.5  & 15.2 & 15.4 & 13.6\\ 
0534302-051148 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 27.1 $\pm$ 3.1  & 0.0 & 0.0 & 5.5\\ 
0534336-051436 & 25.4 $\pm$ 1.2  & 24.8 $\pm$ 1.0  & 26.5 $\pm$ 1.1  & 15.9 & 22.8 & 18.9\\ 
0534359-051524 & -151.3 $\pm$ 3.8  & 25.7 $\pm$ 2.8  & 0.0 $\pm$ 0.0  & 4.2 & 6.2 & 0.0\\ 
0534406-050658 & 32.8 $\pm$ 3.5  & 35.7 $\pm$ 3.8  & 0.0 $\pm$ 0.0  & 4.7 & 4.2 & 0.0\\ 
0534423-051238 & 38.8 $\pm$ 3.0  & -97.5 $\pm$ 4.4  & 0.0 $\pm$ 0.0  & 5.6 & 3.6 & 0.0\\ 
0534424-051218 & 26.1 $\pm$ 1.0  & 25.7 $\pm$ 1.0  & 24.7 $\pm$ 1.0  & 19.9 & 23.1 & 21.2\\ 
0534424-052246 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 34.0 $\pm$ 4.3  & 0.0 & 0.0 & 3.6\\ 
0534429-052006 & 21.3 $\pm$ 1.0  & 21.9 $\pm$ 1.0  & 32.6 $\pm$ 2.5  & 20.5 & 21.3 & 7.1\\ 
0534436-051827 & 14.3 $\pm$ 0.7  & 15.6 $\pm$ 0.8  & 16.7 $\pm$ 0.8  & 35.5 & 30.1 & 31.3\\ 
0534449-050649 & 33.7 $\pm$ 1.6  & 0.0 $\pm$ 0.0  & 31.1 $\pm$ 1.4  & 11.9 & 0.0 & 14.8\\ 
0534450-050620 & 35.5 $\pm$ 3.8  & 29.3 $\pm$ 3.2  & 35.0 $\pm$ 3.0  & 4.3 & 5.4 & 5.8\\ 
0534459-052455 & 18.0 $\pm$ 2.8  & 20.1 $\pm$ 1.8  & 26.1 $\pm$ 2.5  & 6.3 & 10.9 & 7.1\\ 
0534481-052238 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & -29.9 $\pm$ 4.5  & 0.0 & 0.0 & 3.5\\ 
0534482-050713 & 66.7 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 21.8 $\pm$ 2.6  & 3.6 & 0.0 & 6.9\\ 
0534487-051746 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 26.0 $\pm$ 2.8  & 0.0 & 0.0 & 6.1\\ 
0534492-050438 & 25.9 $\pm$ 1.5  & 27.1 $\pm$ 1.4  & 26.0 $\pm$ 1.3  & 13.3 & 14.1 & 15.2\\ 
0534492-051855 & 0.0 $\pm$ 0.0  & 23.4 $\pm$ 3.0  & 41.9 $\pm$ 3.7  & 0.0 & 5.7 & 4.4\\ 
0534504-051110 & 26.7 $\pm$ 1.0  & 27.4 $\pm$ 0.8  & 27.6 $\pm$ 0.8  & 20.1 & 29.0 & 30.2\\ 
0534504-051629 & 25.9 $\pm$ 3.1  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 5.5 & 0.0 & 0.0\\ 
0534506-050407 & 31.6 $\pm$ 1.7  & 33.0 $\pm$ 1.5  & 30.9 $\pm$ 1.6  & 11.3 & 13.2 & 11.8\\ 
0534507-052401 & 20.1 $\pm$ 2.0  & 23.5 $\pm$ 1.4  & 18.0 $\pm$ 2.0  & 9.3 & 14.0 & 9.3\\ 
0534509-051756 & 0.0 $\pm$ 0.0  & 28.3 $\pm$ 2.6  & 0.0 $\pm$ 0.0  & 0.0 & 7.0 & 0.0\\ 
0534514-051329 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 22.1 $\pm$ 4.1  & 0.0 & 0.0 & 3.9\\ 
0534522-051203 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 24.6 $\pm$ 2.0  & 0.0 & 0.0 & 9.4\\ 
0534525-052403 & 21.4 $\pm$ 1.5  & 19.3 $\pm$ 2.0  & 17.5 $\pm$ 2.5  & 12.4 & 9.2 & 7.3\\ 
0534534-051027 & 24.7 $\pm$ 2.4  & 0.0 $\pm$ 0.0  & 22.9 $\pm$ 2.1  & 7.3 & 0.0 & 8.7\\ 
0534537-050548 & 26.0 $\pm$ 1.8  & 27.2 $\pm$ 1.5  & 28.8 $\pm$ 1.4  & 10.7 & 12.7 & 14.8\\ 
0534561-050601 & 48.1 $\pm$ 3.1  & 0.0 $\pm$ 0.0  & 21.8 $\pm$ 3.8  & 5.5 & 0.0 & 4.3\\ 
0534566-051112 & 34.8 $\pm$ 2.6  & 32.7 $\pm$ 3.0  & 37.4 $\pm$ 3.2  & 6.8 & 5.8 & 5.3\\ 
0534580-051737 & 28.0 $\pm$ 2.0  & 30.1 $\pm$ 1.8  & 30.4 $\pm$ 3.4  & 9.1 & 10.8 & 5.0\\ 
0534581-050927 & 21.7 $\pm$ 1.3  & 23.8 $\pm$ 1.2  & 25.1 $\pm$ 1.3  & 15.2 & 17.1 & 15.3\\ 
0534581-051153 & 22.0 $\pm$ 2.3  & 22.1 $\pm$ 2.0  & 22.8 $\pm$ 2.2  & 7.8 & 9.4 & 8.2\\ 
0534593-050530 & 31.6 $\pm$ 2.1  & 0.0 $\pm$ 0.0  & 27.8 $\pm$ 1.6  & 8.7 & 0.0 & 12.3\\ 
0534595-052400 & 27.6 $\pm$ 1.8  & 23.9 $\pm$ 2.1  & 25.3 $\pm$ 3.0  & 10.1 & 8.9 & 5.8\\ 
0535003-050943 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 26.2 $\pm$ 3.4  & 0.0 & 0.0 & 4.9\\ 
0535003-050944 & 24.9 $\pm$ 1.5  & 25.6 $\pm$ 2.5  & 0.0 $\pm$ 0.0  & 12.6 & 7.2 & 0.0\\ 
0535004-052514 & 24.5 $\pm$ 1.9  & 25.9 $\pm$ 1.3  & 23.3 $\pm$ 1.3  & 9.9 & 15.9 & 16.3\\ 
0535006-050508 & 28.3 $\pm$ 1.9  & 21.4 $\pm$ 2.9  & 28.7 $\pm$ 1.5  & 10.1 & 5.9 & 13.6\\ 
0535014-051104 & -127.3 $\pm$ 4.2  & 0.0 $\pm$ 0.0  & -24.2 $\pm$ 3.5  & 3.8 & 0.0 & 4.8\\ 
0535031-050917 & 87.7 $\pm$ 4.1  & 0.0 $\pm$ 0.0  & 36.1 $\pm$ 2.8  & 3.9 & 0.0 & 6.2\\ 
0535031-051829 & 29.9 $\pm$ 2.5  & 28.3 $\pm$ 1.4  & 29.6 $\pm$ 1.8  & 7.1 & 14.8 & 10.4\\ 
0535045-052356 & 29.2 $\pm$ 1.8  & 33.0 $\pm$ 1.8  & 32.3 $\pm$ 2.9  & 10.2 & 10.3 & 6.0\\ 
0535046-050955 & 22.4 $\pm$ 1.4  & 28.2 $\pm$ 1.4  & 53.4 $\pm$ 2.2  & 14.3 & 14.9 & 8.1\\ 
0535047-051742 & -2.0 $\pm$ 3.1  & 25.8 $\pm$ 3.4  & 17.8 $\pm$ 2.5  & 5.5 & 4.9 & 7.1\\ 
0535047-052638 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 21.6 $\pm$ 3.8  & 0.0 & 0.0 & 4.3\\ 
0535051-052024 & 25.9 $\pm$ 2.4  & 25.6 $\pm$ 2.2  & 24.4 $\pm$ 3.6  & 7.6 & 8.2 & 4.7\\ 
0535052-051450 & 54.5 $\pm$ 1.8  & 0.0 $\pm$ 0.0  & 25.4 $\pm$ 1.3  & 10.7 & 0.0 & 15.1\\ 
0535052-052603 & 0.0 $\pm$ 0.0  & 26.1 $\pm$ 4.2  & 0.0 $\pm$ 0.0  & 0.0 & 3.8 & 0.0\\ 
0535054-052717 & 25.9 $\pm$ 1.8  & 27.7 $\pm$ 1.3  & 29.1 $\pm$ 1.4  & 10.2 & 16.2 & 14.6\\ 
0535057-051134 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 11.3 $\pm$ 3.6  & 0.0 & 0.0 & 4.6\\ 
0535057-051135 & 0.0 $\pm$ 0.0  & 177.0 $\pm$ 4.1  & 0.0 $\pm$ 0.0  & 0.0 & 3.9 & 0.0\\ 
0535057-052418 & 191.0 $\pm$ 4.1  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 3.9 & 0.0 & 0.0\\ 
0535057-052626 & 29.0 $\pm$ 2.2  & 31.9 $\pm$ 2.7  & 29.3 $\pm$ 2.9  & 8.3 & 6.6 & 6.0\\ 
0535058-052701 & 25.6 $\pm$ 4.0  & 30.0 $\pm$ 3.3  & 38.8 $\pm$ 4.0  & 4.0 & 5.1 & 4.1\\ 
0535065-051722 & 0.0 $\pm$ 0.0  & 69.6 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 0.0 & 3.7 & 0.0\\ 
0535068-051038 & 36.3 $\pm$ 3.6  & 0.0 $\pm$ 0.0  & -52.9 $\pm$ 3.4  & 4.7 & 0.0 & 5.0\\ 
0535075-051114 & 0.0 $\pm$ 0.0  & 22.5 $\pm$ 2.5  & 20.4 $\pm$ 2.0  & 0.0 & 7.2 & 9.1\\ 
0535087-050440 & 36.6 $\pm$ 3.8  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 4.4 & 0.0 & 0.0\\ 
0535097-052128 & 0.0 $\pm$ 0.0  & 29.6 $\pm$ 4.4  & 0.0 $\pm$ 0.0  & 0.0 & 3.6 & 0.0\\ 
0535103-052113 & 24.2 $\pm$ 2.8  & 30.3 $\pm$ 3.7  & 26.0 $\pm$ 4.0  & 6.2 & 4.5 & 4.0\\ 
0535105-052618 & 21.5 $\pm$ 1.1  & 23.2 $\pm$ 1.0  & 20.7 $\pm$ 1.2  & 19.2 & 20.8 & 16.9\\ 
0535118-052103 & 0.0 $\pm$ 0.0  & -143.6 $\pm$ 4.5  & 0.0 $\pm$ 0.0  & 0.0 & 3.5 & 0.0\\ 
0535119-052033 & 48.4 $\pm$ 3.7  & 31.0 $\pm$ 3.2  & 24.7 $\pm$ 4.1  & 4.5 & 5.3 & 4.0\\ 
0535123-052347 & 28.6 $\pm$ 1.6  & 26.9 $\pm$ 2.7  & 28.1 $\pm$ 1.6  & 11.6 & 6.7 & 11.8\\ 
0535130-051904 & 30.6 $\pm$ 4.4  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 3.5 & 0.0 & 0.0\\ 
0535130-052030 & 0.0 $\pm$ 0.0  & 62.6 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 0.0 & 3.6 & 0.0\\ 
0535134-051710 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 4.5 $\pm$ 4.0  & 0.0 & 0.0 & 4.1\\ 
0535144-051725 & 29.3 $\pm$ 2.4  & 28.2 $\pm$ 3.9  & 32.3 $\pm$ 4.3  & 7.4 & 4.1 & 3.6\\ 
0535146-050852 & 0.0 $\pm$ 0.0  & 22.6 $\pm$ 2.9  & 22.8 $\pm$ 2.7  & 0.0 & 6.1 & 6.7\\ 
0535146-052042 & 18.5 $\pm$ 3.6  & 0.0 $\pm$ 0.0  & -145.3 $\pm$ 4.1  & 4.6 & 0.0 & 4.0\\ 
0535153-051902 & 148.9 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 3.7 & 0.0 & 0.0\\ 
0535153-052215 & 25.1 $\pm$ 1.2  & 19.0 $\pm$ 1.9  & 21.0 $\pm$ 1.9  & 17.0 & 9.9 & 10.1\\ 
0535154-052722 & 25.7 $\pm$ 3.9  & 31.0 $\pm$ 3.2  & 32.8 $\pm$ 4.1  & 4.1 & 5.4 & 3.9\\ 
0535155-052514 & 21.7 $\pm$ 1.4  & 57.1 $\pm$ 3.2  & 37.5 $\pm$ 4.2  & 13.6 & 5.4 & 3.8\\ 
0535156-052533 & 26.3 $\pm$ 4.0  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 4.0 & 0.0 & 0.0\\ 
0535157-052628 & 21.2 $\pm$ 3.9  & 26.7 $\pm$ 3.5  & 0.0 $\pm$ 0.0  & 4.1 & 4.8 & 0.0\\ 
0535159-051657 & 26.4 $\pm$ 2.5  & 31.8 $\pm$ 3.7  & 28.2 $\pm$ 3.5  & 7.1 & 4.5 & 4.8\\ 
0535167-051901 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 13.4 $\pm$ 4.1  & 0.0 & 0.0 & 3.9\\ 
0535171-051239 & 23.6 $\pm$ 2.8  & 35.7 $\pm$ 2.4  & 34.1 $\pm$ 2.7  & 6.2 & 7.6 & 6.6\\ 
0535172-052027 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 23.8 $\pm$ 3.8  & 0.0 & 0.0 & 4.3\\ 
0535172-052316 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 17.3 $\pm$ 4.0  & 0.0 & 0.0 & 4.0\\ 
0535173-052235 & 23.2 $\pm$ 2.5  & 30.7 $\pm$ 4.4  & 0.0 $\pm$ 0.0  & 7.1 & 3.5 & 0.0\\ 
0535175-052256 & 25.4 $\pm$ 1.9  & 27.0 $\pm$ 2.2  & 29.5 $\pm$ 2.0  & 10.1 & 8.5 & 9.4\\ 
0535179-052650 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 29.5 $\pm$ 3.9  & 0.0 & 0.0 & 4.2\\ 
0535180-051546 & 34.7 $\pm$ 3.5  & 52.1 $\pm$ 4.1  & 0.0 $\pm$ 0.0  & 4.8 & 3.9 & 0.0\\ 
0535181-052335 & 24.0 $\pm$ 1.7  & 27.0 $\pm$ 1.6  & 27.1 $\pm$ 2.0  & 11.3 & 11.9 & 9.6\\ 
0535188-051614 & 21.2 $\pm$ 0.8  & 21.0 $\pm$ 1.0  & 21.0 $\pm$ 1.0  & 28.5 & 21.6 & 21.3\\ 
0535196-052426 & 16.7 $\pm$ 3.8  & 0.0 $\pm$ 0.0  & 27.4 $\pm$ 3.0  & 4.3 & 0.0 & 5.8\\ 
0535197-051405 & 28.3 $\pm$ 3.2  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 5.3 & 0.0 & 0.0\\ 
0535200-052105 & 19.5 $\pm$ 2.5  & 21.3 $\pm$ 2.7  & 23.0 $\pm$ 3.3  & 7.0 & 6.6 & 5.1\\ 
0535203-050226 & 26.0 $\pm$ 2.8  & 28.6 $\pm$ 3.2  & 28.7 $\pm$ 2.9  & 6.3 & 5.2 & 6.1\\ 
0535207-052155 & 24.1 $\pm$ 1.4  & 23.0 $\pm$ 3.0  & 22.8 $\pm$ 3.6  & 13.8 & 5.7 & 4.7\\ 
0535214-050903 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 42.7 $\pm$ 3.3  & 0.0 & 0.0 & 5.1\\ 
0535215-050949 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 29.1 $\pm$ 3.5  & 0.0 & 0.0 & 4.7\\ 
0535218-050701 & 25.1 $\pm$ 4.1  & 28.5 $\pm$ 1.1  & 26.7 $\pm$ 1.9  & 3.9 & 19.4 & 10.1\\ 
0535218-052353 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 22.3 $\pm$ 2.7  & 0.0 & 0.0 & 6.5\\ 
0535219-051427 & 23.0 $\pm$ 1.2  & 26.3 $\pm$ 1.3  & 25.6 $\pm$ 1.4  & 16.1 & 16.1 & 14.3\\ 
0535221-052424 & 34.1 $\pm$ 2.4  & 28.9 $\pm$ 1.2  & 78.6 $\pm$ 2.2  & 7.5 & 17.1 & 8.4\\ 
0535222-052029 & 24.1 $\pm$ 0.8  & 20.8 $\pm$ 0.9  & 21.5 $\pm$ 0.9  & 27.5 & 26.9 & 27.6\\ 
0535223-052728 & 0.0 $\pm$ 0.0  & 24.8 $\pm$ 4.1  & 0.0 $\pm$ 0.0  & 0.0 & 3.9 & 0.0\\ 
0535224-050911 & 25.4 $\pm$ 0.9  & 25.9 $\pm$ 1.1  & 26.7 $\pm$ 2.8  & 24.4 & 20.0 & 6.2\\ 
0535226-051411 & 14.7 $\pm$ 2.4  & 21.7 $\pm$ 3.1  & 23.9 $\pm$ 2.7  & 7.5 & 5.5 & 6.4\\ 
0535227-052313 & 23.4 $\pm$ 3.2  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 5.2 & 0.0 & 0.0\\ 
0535234-051051 & 22.5 $\pm$ 1.0  & 22.8 $\pm$ 1.1  & 23.9 $\pm$ 1.1  & 21.3 & 19.5 & 19.5\\ 
0535235-051857 & 9.2 $\pm$ 3.9  & 0.0 $\pm$ 0.0  & 20.1 $\pm$ 2.0  & 4.1 & 0.0 & 9.2\\ 
0535242-052518 & 0.0 $\pm$ 0.0  & 122.4 $\pm$ 4.2  & 29.0 $\pm$ 3.8  & 0.0 & 3.8 & 4.4\\ 
0535244-052439 & 20.1 $\pm$ 3.3  & 21.6 $\pm$ 2.8  & 17.8 $\pm$ 3.5  & 5.1 & 6.2 & 4.8\\ 
0535246-051129 & 0.0 $\pm$ 0.0  & 14.6 $\pm$ 3.7  & -68.8 $\pm$ 3.8  & 0.0 & 4.5 & 4.4\\ 
0535246-051158 & 35.7 $\pm$ 3.7  & -85.8 $\pm$ 4.2  & 26.3 $\pm$ 4.2  & 4.4 & 3.8 & 3.8\\ 
0535246-051909 & -60.3 $\pm$ 4.4  & 0.0 $\pm$ 0.0  & 20.2 $\pm$ 3.9  & 3.6 & 0.0 & 4.2\\ 
0535250-052258 & 25.7 $\pm$ 1.0  & 25.8 $\pm$ 2.0  & 25.6 $\pm$ 1.5  & 21.1 & 9.1 & 12.7\\ 
0535252-050927 & 31.9 $\pm$ 1.8  & 26.5 $\pm$ 2.6  & 27.5 $\pm$ 1.6  & 10.6 & 7.0 & 11.7\\ 
0535253-051048 & 21.4 $\pm$ 0.9  & 21.7 $\pm$ 1.0  & 22.2 $\pm$ 1.0  & 25.3 & 22.0 & 21.7\\ 
0535256-050757 & 31.0 $\pm$ 3.6  & 28.7 $\pm$ 3.9  & 0.0 $\pm$ 0.0  & 4.6 & 4.2 & 0.0\\ 
0535260-050837 & 25.3 $\pm$ 2.3  & 31.9 $\pm$ 2.2  & 27.3 $\pm$ 2.0  & 7.9 & 8.5 & 9.2\\ 
0535268-051107 & 20.3 $\pm$ 1.1  & 0.0 $\pm$ 0.0  & 25.4 $\pm$ 1.2  & 19.1 & 0.0 & 17.3\\ 
0535274-051709 & 26.4 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 9.1 $\pm$ 3.3  & 3.7 & 0.0 & 5.2\\ 
0535274-052628 & 29.4 $\pm$ 1.3  & 22.8 $\pm$ 1.1  & 29.9 $\pm$ 1.5  & 15.2 & 18.4 & 13.6\\ 
0535281-051013 & -78.2 $\pm$ 4.1  & 20.6 $\pm$ 4.0  & 0.0 $\pm$ 0.0  & 4.0 & 4.1 & 0.0\\ 
0535281-051014 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 21.5 $\pm$ 2.6  & 0.0 & 0.0 & 6.9\\ 
0535281-052134 & 192.5 $\pm$ 4.4  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 3.5 & 0.0 & 0.0\\ 
0535290-050604 & 28.4 $\pm$ 0.8  & 30.6 $\pm$ 1.2  & 30.6 $\pm$ 1.1  & 27.5 & 17.9 & 19.7\\ 
0535293-052546 & 23.6 $\pm$ 2.4  & 23.7 $\pm$ 3.1  & 0.0 $\pm$ 0.0  & 7.4 & 5.5 & 0.0\\ 
0535298-051210 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & -1.5 $\pm$ 4.0  & 0.0 & 0.0 & 4.1\\ 
0535298-052355 & 28.0 $\pm$ 1.9  & 27.3 $\pm$ 1.3  & 23.5 $\pm$ 2.0  & 9.7 & 15.2 & 9.3\\ 
0535304-052423 & 8.1 $\pm$ 4.5  & 38.0 $\pm$ 4.3  & 29.1 $\pm$ 3.0  & 3.5 & 3.7 & 5.8\\ 
0535304-052538 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 23.3 $\pm$ 2.3  & 0.0 & 0.0 & 7.7\\ 
0535306-051516 & 28.8 $\pm$ 2.3  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 8.0 & 0.0 & 0.0\\ 
0535307-051807 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & -62.9 $\pm$ 3.9  & 0.0 & 0.0 & 4.1\\ 
0535312-051533 & 26.3 $\pm$ 0.8  & 26.7 $\pm$ 1.1  & 27.8 $\pm$ 1.3  & 26.5 & 18.7 & 16.4\\ 
0535312-052340 & 23.2 $\pm$ 4.2  & 0.0 $\pm$ 0.0  & 23.8 $\pm$ 1.4  & 3.8 & 0.0 & 13.9\\ 
0535314-050501 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & -76.5 $\pm$ 3.5  & 0.0 & 0.0 & 4.8\\ 
0535314-052516 & 0.0 $\pm$ 0.0  & 25.3 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 0.0 & 3.6 & 0.0\\ 
0535316-051636 & 0.0 $\pm$ 0.0  & -59.4 $\pm$ 4.3  & 0.0 $\pm$ 0.0  & 0.0 & 3.7 & 0.0\\ 
0535319-050927 & 26.5 $\pm$ 1.1  & 73.8 $\pm$ 4.0  & 0.0 $\pm$ 0.0  & 17.9 & 4.0 & 0.0\\ 
0535319-050928 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 27.4 $\pm$ 1.2  & 0.0 & 0.0 & 17.8\\ 
0535321-051157 & 0.0 $\pm$ 0.0  & -67.5 $\pm$ 4.5  & 16.7 $\pm$ 3.7  & 0.0 & 3.5 & 4.5\\ 
0535323-051807 & 0.0 $\pm$ 0.0  & 28.5 $\pm$ 2.6  & 35.8 $\pm$ 2.7  & 0.0 & 6.7 & 6.5\\ 
0535324-051424 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 21.5 $\pm$ 3.7  & 0.0 & 0.0 & 4.5\\ 
0535324-051506 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 30.5 $\pm$ 4.2  & 0.0 & 0.0 & 3.8\\ 
0535325-052610 & 16.7 $\pm$ 4.0  & 20.0 $\pm$ 4.4  & 34.4 $\pm$ 3.4  & 4.1 & 3.6 & 4.9\\ 
0535329-051605 & 29.3 $\pm$ 1.5  & 26.9 $\pm$ 2.0  & 29.8 $\pm$ 2.4  & 13.3 & 9.6 & 7.6\\ 
0535353-050846 & 25.0 $\pm$ 2.8  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 6.1 & 0.0 & 0.0\\ 
0535353-051111 & 28.8 $\pm$ 2.8  & 28.5 $\pm$ 3.3  & 25.2 $\pm$ 3.0  & 6.2 & 5.1 & 5.7\\ 
0535355-050658 & 26.4 $\pm$ 1.3  & 28.1 $\pm$ 1.5  & 28.5 $\pm$ 1.3  & 15.6 & 13.1 & 16.2\\ 
0535359-051225 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & -102.0 $\pm$ 4.0  & 0.0 & 0.0 & 4.0\\ 
0535360-051225 & 23.3 $\pm$ 3.9  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 4.2 & 0.0 & 0.0\\ 
0535366-050414 & 0.0 $\pm$ 0.0  & 23.5 $\pm$ 3.6  & 27.6 $\pm$ 1.8  & 0.0 & 4.6 & 10.5\\ 
0535367-051000 & 28.1 $\pm$ 3.0  & 120.9 $\pm$ 4.4  & 0.0 $\pm$ 0.0  & 5.8 & 3.5 & 0.0\\ 
0535371-051029 & 30.1 $\pm$ 1.1  & 29.9 $\pm$ 1.4  & 30.2 $\pm$ 1.3  & 18.2 & 14.9 & 15.0\\ 
0535376-050632 & 28.7 $\pm$ 4.1  & 0.0 $\pm$ 0.0  & -74.4 $\pm$ 3.7  & 3.9 & 0.0 & 4.5\\ 
0535387-051659 & 26.7 $\pm$ 2.3  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 7.8 & 0.0 & 0.0\\ 
0535388-051241 & 23.5 $\pm$ 1.9  & 45.7 $\pm$ 3.1  & 0.0 $\pm$ 0.0  & 9.6 & 5.5 & 0.0\\ 
0535388-051242 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 30.5 $\pm$ 1.6  & 0.0 & 0.0 & 12.0\\ 
0535390-050704 & 20.1 $\pm$ 1.8  & 20.3 $\pm$ 1.6  & 25.3 $\pm$ 1.7  & 10.1 & 12.2 & 11.6\\ 
0535390-050856 & 30.0 $\pm$ 3.3  & 20.0 $\pm$ 2.8  & 11.3 $\pm$ 2.1  & 5.1 & 6.3 & 8.9\\ 
0535399-050636 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 25.4 $\pm$ 4.0  & 0.0 & 0.0 & 4.1\\ 
0535401-051729 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & -172.0 $\pm$ 4.3  & 0.0 & 0.0 & 3.7\\ 
0535406-051219 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 14.9 $\pm$ 4.4  & 0.0 & 0.0 & 3.6\\ 
0535410-050625 & 27.1 $\pm$ 3.2  & 0.0 $\pm$ 0.0  & 28.6 $\pm$ 2.5  & 5.3 & 0.0 & 7.2\\ 
0535420-051011 & 0.0 $\pm$ 0.0  & 192.9 $\pm$ 3.7  & 33.5 $\pm$ 4.1  & 0.0 & 4.5 & 3.9\\ 
0535420-051259 & 26.7 $\pm$ 3.6  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 4.6 & 0.0 & 0.0\\ 
0535423-051508 & 25.5 $\pm$ 3.6  & 0.0 $\pm$ 0.0  & -19.5 $\pm$ 3.8  & 4.5 & 0.0 & 4.3\\ 
0535427-051154 & 8.4 $\pm$ 2.2  & 23.6 $\pm$ 2.4  & 26.7 $\pm$ 2.5  & 8.3 & 7.4 & 7.2\\ 
0535432-050917 & 24.9 $\pm$ 2.7  & 14.4 $\pm$ 2.1  & 10.6 $\pm$ 2.2  & 6.4 & 8.6 & 8.5\\ 
0535435-050541 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 27.9 $\pm$ 2.5  & 0.0 & 0.0 & 7.1\\ 
0535437-050958 & 28.3 $\pm$ 3.2  & 29.9 $\pm$ 2.9  & 0.0 $\pm$ 0.0  & 5.2 & 6.0 & 0.0\\ 
0535438-050959 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 29.9 $\pm$ 3.2  & 0.0 & 0.0 & 5.3\\ 
0535445-050731 & 23.2 $\pm$ 3.5  & 0.0 $\pm$ 0.0  & 20.2 $\pm$ 1.7  & 4.7 & 0.0 & 11.0\\ 
0535460-051749 & 28.9 $\pm$ 2.6  & 26.8 $\pm$ 3.4  & 25.3 $\pm$ 2.9  & 6.7 & 4.9 & 5.9\\ 
0535461-051051 & 27.3 $\pm$ 1.6  & 0.0 $\pm$ 0.0  & 19.4 $\pm$ 1.4  & 11.7 & 0.0 & 13.7\\ 
0535462-051539 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 34.4 $\pm$ 3.4  & 0.0 & 0.0 & 4.9\\ 
0535462-051808 & 25.9 $\pm$ 3.6  & 0.0 $\pm$ 0.0  & 30.3 $\pm$ 1.7  & 4.5 & 0.0 & 11.2\\ 
0535474-051028 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 24.4 $\pm$ 2.7  & 0.0 & 0.0 & 6.6\\ 
0535475-051658 & 2.1 $\pm$ 0.7  & 4.9 $\pm$ 0.9  & 4.6 $\pm$ 0.9  & 31.4 & 25.2 & 25.7\\ 
0535478-051317 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 14.6 $\pm$ 4.3  & 0.0 & 0.0 & 3.7\\ 
0535482-051110 & 27.4 $\pm$ 3.5  & 0.0 $\pm$ 0.0  & 21.8 $\pm$ 3.5  & 4.8 & 0.0 & 4.8\\ 
0535490-051537 & 27.6 $\pm$ 1.4  & 28.4 $\pm$ 1.5  & 29.8 $\pm$ 1.5  & 13.5 & 13.3 & 13.4\\ 
0535498-051830 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 14.9 $\pm$ 4.3  & 0.0 & 0.0 & 3.6\\ 
0535507-051629 & 17.6 $\pm$ 2.6  & 0.0 $\pm$ 0.0  & 26.8 $\pm$ 1.6  & 6.8 & 0.0 & 11.8\\ 
0535510-051509 & 27.0 $\pm$ 1.5  & 0.0 $\pm$ 0.0  & 25.1 $\pm$ 1.6  & 12.5 & 0.0 & 12.6\\ 
0535511-050708 & 27.8 $\pm$ 3.6  & 0.0 $\pm$ 0.0  & 26.6 $\pm$ 1.7  & 4.7 & 0.0 & 11.2\\ 
0535527-051259 & 29.7 $\pm$ 1.5  & 0.0 $\pm$ 0.0  & 27.6 $\pm$ 1.4  & 12.7 & 0.0 & 14.1\\ 
0535541-051710 & 0.0 $\pm$ 0.0  & 25.5 $\pm$ 3.1  & 43.9 $\pm$ 3.9  & 0.0 & 5.5 & 4.1\\ 
0535546-052200 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 24.1 $\pm$ 4.0  & 0.0 & 0.0 & 4.0\\ 
0535547-051055 & 38.4 $\pm$ 0.7  & 38.0 $\pm$ 1.2  & 37.5 $\pm$ 1.0  & 35.4 & 17.1 & 22.3\\ 
0535549-051315 & 64.6 $\pm$ 1.2  & 0.0 $\pm$ 0.0  & 63.3 $\pm$ 1.8  & 16.7 & 0.0 & 10.8\\ 
0535568-051957 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 69.5 $\pm$ 3.8  & 0.0 & 0.0 & 4.3\\ 
0536013-051910 & 26.5 $\pm$ 2.2  & 24.0 $\pm$ 1.8  & 29.0 $\pm$ 2.6  & 8.1 & 10.8 & 6.9\\ 
0536027-051526 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 16.6 $\pm$ 3.2  & 0.0 & 0.0 & 5.3\\ 
\enddata
\end{deluxetable}

